Fragmentation Considered Poisonous

We present practical poisoning and name-server block- ing attacks on standard DNS resolvers, by off-path, spoofing adversaries. Our attacks exploit large DNS responses that cause IP fragmentation; such long re- sponses are increasingly common, mainly due to the use of DNSSEC. In common scenarios, where DNSSEC is partially or incorrectly deployed, our poisoning attacks allow 'com- plete' domain hijacking. When DNSSEC is fully de- ployed, attacker can force use of fake name server; we show exploits of this allowing off-path traffic analy- sis and covert channel. When using NSEC3 opt-out, attacker can also create fake subdomains, circumvent- ing same origin restrictions. Our attacks circumvent resolver-side defenses, e.g., port randomisation, IP ran- domisation and query randomisation. The (new) name server (NS) blocking attacks force re- solver to use specific name server. This attack allows Degradation of Service, traffic-analysis and covert chan- nel, and also facilitates DNS poisoning. We validated the attacks using standard resolver soft- ware and standard DNS name servers and zones, e.g., org.

==> abstract.tex <==
\begin{abstract}
We present practical {\em poisoning} and {\em name-server blocking} attacks on standard DNS resolvers, by {\em off-path, spoofing adversaries}. 
Our attacks exploit large DNS responses that cause IP fragmentation; such long responses are increasingly common, mainly due to the use of DNSSEC. 

In common scenarios, where DNSSEC is partially or incorrectly deployed, our poisoning attacks allow `complete' domain hijacking. When DNSSEC is fully deployed, attacker can  force use of fake name server; we show exploits of this allowing off-path traffic analysis and covert channel. When using NSEC3 opt-out, attacker can also create fake subdomains, circumventing same origin restrictions. 
Our attacks 
%extend Kaminsky's cache poisoning attack \cite{Kaminsky08}, improving its effectiveness and circumventing the known (and effective) 
circumvent resolver-side defenses, e.g.,  port randomisation, IP randomisation and query randomisation. 

%We show how this allows off-path DNS poisoning, in common scenarios where DNSSEC is not (fully and correctly) used, e.g., due to interoperability and other deployment challenges. Our techniques also allow an off-path attacker to poison the DNS response with a mapping to a non-existing subdomain, even when DNSSEC is fully deployed, but the zone uses NSEC3 opt-out.

%We also show off-path poisoning of resolver with a mapping to a non-existing subdomain, even when DNSSEC is fully deployed, when using NSEC3 with opt-out. 

%The attack circumvent existing and proposed on-crypt This allows attackers to perform effective poisoning, bypassing the (so far effective) `patches', as well as {\em off-path name server hijacking}, which we identify as a significant threat.  

%These attacks fail, in the (currently less common) case where DNSSEC is fully and correctly deployed. 
%Our server-forcing attacks apply even for full, correct use of DNSSEC. The {\em DoS attacks} allow efficient disabling of DNS services. We present two variants: one for all resolvers, and an even more efficient one for resolvers that follow RFC4697 \cite{rfc4697}.  
 
The (new) {\em name server (NS) blocking} attacks force resolver to use specific name server. This attack allows {\em Degradation of Service, traffic-analysis and covert channel}, and also facilitates DNS poisoning. 

We validated the attacks using standard resolver software and standard DNS name servers and zones, e.g., {\sf org}.
\end{abstract}
% should we mention requirments of attacks? and variant abusing Matt RFC to cause `NS selection` and thereby Denial/degradation, traffic analysis and even poisoning (via vulnerable server), even when 2nd frag isn't usable to do NS poisoning? 
%In {\em NS poisoning}, resolvers cache fake NS (name server) records, and use them instead of the correct NS records. 
%We clarify the res
%
%It was known that MitM attackers can change name servers of child domains in referrals, evan using DNSSEC; we show that this can be extended to a new significant threat: {\em name server hijacking}, allowing Furthermore, we show how off-path attackers can perform these attacks. 
%
%We validated the attacks over the Internet, against the name servers of TLDs, and using popular resolvers. 

%Actually there are libraries 

%This is an early disclosure of a {\sf vulnerability} due to the use of  allowing efficient poisoning of recursive DNS resolvers}, as well as DoS attack, preventing resolution of victim domains. The vulnerability is due to {\em fragmentation} of DNS responses, e.g., as a result of the use of DNSSEC RRs, and allows {\em cache poisoning} and {\em denial of service} attacks by off-path (blind) spoofing adversaries, on recursive DNS resolvers. Our attacks are efficient since they do not require guessing the UDP source port, the DNS transaction ID selected by the resolver, and also circumvent the protection offered by other DNS mechanisms, e.g., DNS 0x20 encoding.

%{\sc Cache poisoning attacks}: fragmentation of DNS responses allows poisoning the entries of recursive DNS resolvers for domains that do not support DNSSEC, but whose parent does, e.g., the children of most top level domains. Note that the vulnerability does {\em not} break the security of DNSSEC itself, and it only exploits the fragmentation due to large DNSSEC enabled DNS responses.
%We also show that attackers can inflict fragmentation of DNS responses, even when they are significantly smaller than $1500$ bytes, by spoofing an ICMP fragmentation needed packets. This allows poisoning of {\em any} DNS response, that is larger than 512 bytes. 

%In the course of our study, we observed that some recursive resolvers do not strictly implement DNSSEC, e.g., may accept and cache the response even if some signatures are missing. We also show attacks on such resolvers, motivating strict compliance with the recommendations of RFC 4035, to prevent attacks against such resolvers.

%{\sc Denial of service attacks}: we show that when DNS response gets fragmented, a spoofer can deprive the clients of DNS service by sending a forged fragment (often a few or a single fragments suffice). 

%We include a brief description of some of our experimental validation.


%The vulnerability pertains to specification problems in IP and DNS, and seems to work for most or all DNS implementations, and to allow poisoning of many domains. %Some scenarios were already confirmed experimentally, and we are working on testing other scenarios. 

%This manuscript is a draft version intended for early disclosure, to solicit feedback and help coordinate measures to defend Internet users from abuse of this vulnerability. More details will be provided in the full paper.
%, soon to be available from the authors. While we appreciate any feedback, please notice this is not yet even a draft of the paper, in particular, we still have to add much more on previous and related works - many citations still missing; we also do not yet explain {\em why} DNS poisoning is a significant threat. %did not yet discuss related works. 

%Due to the sensitivity, readers are requested not to share this manuscript, except with relevant, trustworthy experts and with authors consent. 


==> defenses.tex <==
\section{Conclusions and Defenses} \label{s:defenses}
We showed how an off-path attacker can efficiently exploit fragmented DNS responses to poison DNS caches. Most DNS responses are short, and hence not fragmented; our attacks exploit DNSSEC records, which often result in fragmented responses. 

We also showed that fragmented responses can be exploited by off-path attackers to force the resolvers to query name servers of attacker's choice.

The attacks are effective against valid implementation of the DNS and IP specifications; furthermore, we have confirmed effectiveness against several domains, using real network scenarios and common resolvers (Unbound 1.4.1 and Bind9).
%Unbound (in addition to strict DNSSEC validation) also supports a `permissive mode' of DNSSEC validation, i.e., if some signatures are missing it may still cache the result, e.g., to ensure functionality in face of devices which are not compliant with DNSSEC, e.g., proxy resolvers, firewalls.
%Note poisoning of the A RR for the afilias name server, as in Figure~\ref{fig:forged:resp:info}, should not be possible with resolvers that correctly enforce DNSSEC validation, e.g., Bind9.

%However, we emphasise that even resolvers that enforce and correctly perform DNSSEC validation are vulnerable to poisoning attacks on domains which are {\em not} protected with DNSSEC, when the DNS responses get fragmented.

We want to caution against drawing the conclusion that DNSSEC should not be used. In fact, the best defense %against the poisoning attacks we described,
is to apply DNSSEC correctly in {\em all} resolvers and domains (without using NSEC3 opt-out); this will certainly prevent many of our poisoning attacks, and even defend against more powerful Man-in-the-Middle adversaries. 
However, incremental DNSSEC deployment is vulnerable to our cache poisoning attacks, and complete adoption of DNSSEC may take considerable time, since it depends on adoption by both name server and resolver. Furthermore, this will not prevent the server blocking attacks. Hence, we also discuss some other defenses, which can be utilised by only one of the parties (unilaterally), and can also prevent the DNS response blocking attacks. 

The vulnerability which allowed us to launch the poisoning attacks against recursive resolvers, is due to the fact that the resolver advertises a large EDNS buffer, which is usually larger than the MTU, e.g., 1500 bytes. Although support of large DNS responses is critical to facilitate DNSSEC enabled DNS responses, or public-key certificates~\cite{cert:dns}, such long responses can be (temporarily) sent over TCP, using path MTU discovery and avoiding fragmentation - unfortunately, at significant performance costs. Another countermeasure, possible at resolver, name server or even at intermediate gateway (firewall), is to set a maximal EDNS buffer value to at most 1500, or even less, to avoid fragmentation. %With respect to DNSSEC this means effectively setting the {\sc do} bit always to 0, i.e., no support of DNSSEC. We also recommend not to allow DNS responses longer than 512 bytes, e.g., public-key certificates.
%This short term defense %, relevant to DNSSEC, 
%can be configured at the resolvers, name servers .
In fact, resolvers may implement a simple protocol similar to path MTU discovery, then set the value of the EDNS buffer accordingly to the minimal MTU en route between the resolver and the DNS server. %The PMTU discovery will allow the resolvers to find out the maximal packet length that can be used for the responses of the name server without causing fragmentation, and this value should be signaled by the resolver in the EDNS RR. 
When sending responses, the name server should also set the DF bit in the IP header to 1, i.e., do not fragment.
 

%Similarly, a short-term countermeasure at the name servers is to bound the legth of EDNS responses by the perceived minimal path MTU (e.g., 1500 bytes), even if resolvers advertise larger EDNS buffers. %and to always send packets with length of verride the EDNS value to at most 1500 bytes.

Another short-term defense, which administrators of resolvers can apply, is to reduce the maximal number of fragments cached; e.g.,  currently 64 by default in Linux (per (source IP , dest IP , protocol) triplet). Of course, reduction in this parameter may also increase packet loss. % Changing to better-randomised choice of IP-ID would also help (but not too much). 



%We caution, however, that such short-term `patching' may remain after better corrective measures were applied, and cause different connectivity and performance problems; hence, other solutions may be preferable. 

%This can also be configured in firewalls, i.e., to set the EDNS to at most 1500 bytes. %Other, non-DNSSEC RRs, which result in long DNS responses, e.g., public-key certificates, should not be supported, e.g., by blocking EDNS in firewall, or by disabling it at the resolver.

Yet another possible defense for name servers, is to always add a {\em random RR} to any packet over certain size (i.e., which may be fragmented). A simple type {\sf A} resource record, containing random IP address for some fictitious domain name, would suffice. The TTL of such an RR should be set to zero to prevent the resolver from caching that record. This would prevent the attacker from being able to predict and (correctly) adjust the checksum value. If there are multiple vulnerable fragments, such a random RR should appear in each fragment. 

Finally, we suggest to be careful when deploying the proposal in \cite{rfc4697,203} (for server selection) which recommends to avoid querying non-responsive servers. Resolvers that do not conform to that recommendation, e.g., Bind9, are not vulnerable to our server-pinning attacks.


==> introduction.tex <==
\section{Introduction}
The correctness and availability of information in the Domain Name System are crucial for the operation of the Internet. 
%This motivated many researchers to identify DNS vulnerabilities, and to develop secure mechanisms. 
In particular, DNS poisoning is a significant threat to Internet security, and can be used for phishing, credentials stealing (e.g., XSS), sending spam and phishing emails, eavesdropping, and more. 
Due to its wide use and universal availability, the DNS is also abused in other ways for different goals, including Denial of Service, fast-flux, covert botnet communication, and more. 

%Furthermore, the correctness and availability of DNS are crucial for security applications that use DNS, e.g., automated  software update services, SPF, DKIM and DNS-stored public-key certificates~\cite{cert:dns}. % and pk cert proposals... add, also citations

Most DNS (poisoning and other) attacks `in the wild', as well as most research, considered an {\em off-path adversary} that is able to send spoofed packets (but not to intercept, modify or block packets). The most well known is Kaminsky's DNS poisoning attack \cite{Kaminsky08}, which was exceedingly effective against many resolvers at the time (2008). Kaminsky's attack, and most other known DNS poisoning attacks, allows the attacker to cause resolvers to provide incorrect (poisoned) responses to DNS queries of the clients, and thereby `hijack' a domain name. We refer to this type of attack as {\em Domain-hijacking DNS poisoning}, to distinguish between it and two other variants of DNS poisoning, to which we also present off-path attacks; more below (and see Table \ref{attacks:table}). 

The increased awareness to the risks of DNS poisoning, following the publication of Kaminsky's attack, was one of the factors helping to speed-up the (long-overdue) adoption of the DNSSEC standard \cite{rfc4035,rfc4034,rfc4033}. DNSSEC uses digital signatures to prevent poisoning of the DNS responses, and is hence secure even against man-in-the-middle (MitM) adversaries. DNSSEC had a long and thorough design and evaluation process, and its security is based on extensive evaluation by many experts, as well as on results of formal analysis, e.g., by Bau and Mitchell \cite{bau2010security}. (There are also alternate proposals for security against MitM, e.g., DNS Curve \cite{DNSCurve}). 

However, deployment of DNSSEC is challenging and would take considerable time. Hence, as a more immediate response to Kaminsky's attack, resolvers were rapidly `patched' to protect against it, mostly following RFC5452 \cite{rfc5452}. The `patches' include {\em source port randomisation, source and destination IP randomisation}, and {\em query randomisation: case toggling} (`0x20 encoding', \cite{DagonAVJL08}) and addition of a {\em random prefix} to queries \cite{DBLP:conf/dsn/PerdisciALL09}. 

These `patches' increase the entropy of `unpredictable' fields copied from DNS requests to DNS responses, and hence are trivially insecure against MitM attackers. However, these patches are considered `best practice', since they are believed to  provide sufficient security against off-path attackers (which is considered as sufficient defenses for many systems). 

We show that, under common scenarios - which seem likely to become even more common in the future, an off-path attacker can efficiently circumvent all of these mechanisms. Namely, an off-path attacker can perform effective `domain-hijacking' DNS poisoning attack, circumventing all the `patches', and with even better efficiency than Kaminsky's poisoning technique. However, our domain-hijacking attack fails when DNSSEC is correctly and fully deployed. This attack works in scenarios where DNSSEC is partially or incorrectly deployed, such as permissive resolvers and islands of trust; currently, such scenarios are rather common. 

%%% macros for names of requirements

\begin{table*}
\begin{center}
\begin{tabular}{|l|l|l|l|l|}
\hline 
\multicolumn{1}{|r|}{Attacks} & \multicolumn{3}{c|}{DNS Poisoning (Section~\ref{sc:poisoning})}  &  Name  Server\\ \cline{2-4}
%       & \multicolumn{2}{c|}{Domain Hijacking} & \multicolumn{2}{c|}{New Subdomain} & Block & Poison \\ \cline{2-5}
 & {Domain Hijacking} & Subdomain Injection & NS Hijacking & Blocking \\\cline{2-5}
Requirements   & Section~\ref{sc:DomHij} &  Section~\ref{sc:SubInj} & Section~\ref{sc:NSInj} & Section~\ref{sc:ns:selection} \\ \hline \hline
%1. $\begin{array}{ll}\textrm{PR or}\\ \textrm {Island} \end{array}$ & $\surd$ & $\surd$ & & & & \\ \hline
IP-ID & $\surd$&  $\surd$& $\surd$   & $\surd$ \\ \hline
\Rfz & $\surd$&  $\surd$& $\surd$   & $\surd$ \\ \hline
\Rpz  & $\surd$  &  $\surd$ & $\surd$& \\ \hline 
\Rdnssec %\Rpr\ or \Ri 
  & $\surd$  & & & \\ \hline
%3. Additional Section &  & $\surd$ & &    & $\surd$\\ \hline
%$\begin{array}{ll} \textrm{NoNX or}\\ \textrm {IgnoreNX} \end{array}$ & $\surd$ & & $\surd$  & & & \\ \hline 
\Ropt  & & $\surd$ &  & \\ \hline
%5. NXD-Frag & & & & & $\surd$ & $\surd$ \\ \hline
RFC 4697 & & & &  $\surd$  \\ \hline
\end{tabular}
\end{center}
\caption{\footnotesize{Our attacks and requirements.}}
\label{attacks:table}
\end{table*}

We also present three other attacks, which apply even if DNSSEC is correctly and universally deployed: %. Two of these are special forms of DNS poisoning attacks: 
%\begin{description}
\paragraph{Subdomain Injection,}
%\item[Subdomain Injection,] 
is a poisoning attack which causes resolvers to accept, cache and provide to clients a mapping for a non-existing (child) domain, of a DNSSEC-protected parent domain. As~\cite{bau2010security} observed, when the parent zone supports NSEC3 opt-out, the attacker can create fake (non-existing) sub-domains; this can lead to attacks on Same Origin Policy such as XSS, phishing and cookie stealing. We show how an off-path attacker can achieve the same effect.
\paragraph{Name Server (NS) Hijacking,} 
is a poisoning attack which causes resolvers to cache and use incorrect name servers for a DNSSEC-protected domain, typically, pointing them to name servers belonging  to the attacker. We show how this attack provides new, efficient off-path methods for traffic analysis, covert channels and Denial of Service; notice the attack and its applications are viable, even if DNSSEC is universally and correctly deployed, since the delegation NS and A resource records (RRs) are not signed.
%Previously, Bernstein pointed out this vulnerability of DNSSEC, but only to point out that DNSSEC does not prevent such attack on unprotected child domains \cite{Bernstein:woot,bau2010security}. 
% can  be exploited for traffic analysis, DoS, and off-path covert channel. 
\paragraph{Name Server (NS) Blocking,} allows the attacker to force resolvers to query name servers of his choice, and stop using other name servers, by corrupting fragmented responses from those name servers. This is not a poisoning attack, since it does not involve a resolver accepting fake resource records. In fact, one application of this attack is to {\em facilitate poisoning}, by causing resolvers to use specific name servers, possibly known to be vulnerable; this provides an effective mechanism to deploy the attack of \cite{ramasubramanian2005perils}, which was, so far, considered impractical. Under certain situations, this attack can also be used for off-path Degradation of Service and traffic analysis.
%\end{description}

%These variants allow exploits including  %Furthermore, while our poisoning attack fails if DNSSEC \cite{rfc4035,rfc4034,rfc4033} is correctly and fully deployed, the other exploits work even if DNSSEC is deployed. 

We summarise all our attacks, with their requirements, in Table \ref{attacks:table}. The requirements are explained in Section \ref{sc:requirements}; for now, it suffices to mention that they all reflect common situations in the current DNS, many of which are not expected to change, even if DNSSEC is fully, universally and correctly deployed. The main exception is attacks which require partial or incorrect DNSSEC deployment; however, not only is this requirement currently often satisfied, but it is also required only for the `domain hijacking' attack. 

In fact, ironically, the use of DNSSEC is often what provides necessary requirements for our attacks to work. Specifically, all of our attacks require {\em \Rfz}, implying fragmented DNS responses; and three of the attacks require {\em \Rpz}, implying that the second fragment contains complete resource record(s), from the `authority' and/or `additional' sections. More details on the requirements are presented within. 

DNSSEC requires long resource records (RRs) which results in long DNS responses. Long DNS responses (i.e., above 512 byte) require support of the EDNS extension mechanism, \cite{rfc2671}, and often fragmented when sent over UDP, since their size exceeds the path MTU. It is exactly this fragmentation that facilitates our attacks; e.g., we show that off-path attackers can often replace the second fragment of a packet, resulting in a seemingly-valid, yet fake, DNS response, or `merely' causing corruption of the DNS response. 

%,Our poisoning attacks require not merely fragmented DNS responses, but an existence of complete resource record(s) in the second fragment. Often, even when DNSSEC is used, the second fragment is not sufficiently long, and may not be long for the domain which attacker wishes to poison. 
%However, as DNSSEC is used more and more, the length of responses is expected to increase (e.g., due to adoption of longer and more keys), increasing vulnerability - unless proper precautions are taken (see Section \ref{s:defenses}). 

%Our DNS poisoning attacks are launched by off-path attackers and deploying cryptographic defenses on resolvers and zones correctly, could foil them, and even attacks by stronger MitM adversaries. Specifically, such strong defenses are possible using the DNSSEC standard, which uses digital signatures to prevent poisoning of the DNS responses by man-in-the-middle (MitM) and weaker adversaries \cite{rfc4035,rfc4034,rfc4033}. DNSSEC was designed more than 15 years ago, and its security is based on extensive evaluation by many experts, as well as on results of formal analysis, e.g., by Bau and Mitchell \cite{bau2010security}. (There are also alternate proposals such as DNS Curve \cite{DNSCurve}). 

%Indeed, while further `patching' may offer interim defenses against our attacks, similarly to the way the currently-deployed patches defend against Kaminsky's original attack, a much better (but possibly longer-term) solution is to adopt cryptographic, MitM-secure mechanisms such as DNSSEC. 
%However, the use of DNSSEC requires long resource records (RRs) which results in long DNS responses. Long DNS responses (i.e., above 512 byte) require support of the EDNS extension mechanism, \cite{rfc2671}, and often fragmented when sent over UDP, since their size exceeds the path MTU. 
%Ironically, it is exactly this fragmentation that facilitates our attacks; specifically, we show that off-path attackers can often replace the second fragment of a packet, resulting in a seemingly-valid, yet fake, DNS response. 

Fragmentation is known to be problematic or `harmful', mainly due to the negative impact on performance; see the seminal paper of Kent and Mogul \cite{KenMog87}. As a result, fragmentation is usually avoided, e.g., by use of path MTU discovery \cite{rfc1191,rfc4821}, mainly for connection-based transport protocol (TCP). 
However, DNS traffic is usually sent over UDP; while several significant name servers, e.g., {\sf com, edu}, send long responses over TCP, this may not be a good long-term solution, since the use of TCP results in significant overhead. 

%{\bf update rest of intro...}
%
%There are common scenarios where the deployment of DNSSEC is incomplete or incorrect, mainly due to concerns about interoperability. The main reasons are {\em permissive resolvers} and {\em islands of security}. For details, see Section~\ref{sc:conditions}.

%When DNSSEC is used correctly, by resolvers and name servers, our `domain hijacking' DNS poisoning attacks fail. 
%However, w

%While correct and complete deployment of DNSSEC prevents Kaminsky style~\cite{kaminsky:dns} DNS poisoning, we show that an off-path attacker can still poison NS (name server) records; this was known before, but only for MitM attackers \cite{Bernstein:woot,bau2010security}. When a zone supports NSEC3 opt-out, the attacker can create fake (non-existing) sub-domains; this can lead to attacks on Same Origin Policy such as XSS, phishing and cookie stealing. Our techniques improve the attack from~\cite{bau2010security} as they require only off-path attacker, instead of a much stronger MitM attacker. 



%Furthermore, we present a new off-path attack we term {\em name server (NS) pinning}, whereby an attacker causes a resolver to direct all or most of its DNS request for some victim zone, towards a particular name server, which may even be a fake name server controlled by the attacker. Server pinning can be used to direct DNS requests towards a compromised name server, e.g., for poisoning, as well as for denial/degradation of service, traffic analysis and covert channel. A summary of our attacks is in Table~\ref{attacks:table}. 

%When the second fragment size does not suffice for poisoning, or when DNSSEC is fully and correctly deployed, we present a different novel attack, which can allow us to trick resolvers into not using certain name servers; this can result in Denial/Degradation of Service, and even in poisoning (by forcing the resolver to use a vulnerable name server). 



%
%However, %DNSSEC but adoption is slow; 
%the vast majority of domains are not yet DNSSEC protected.
%DNSSEC adoption accelerated following Kaminsky's attack \cite{Kaminsky08}, and further after the root and most top-level domains were (recently) signed, but adoption is still slower than desired, with only a fraction of the subdomains deploying DNSSEC. Currently, DNSSEC deployment is significantly advanced in the {\tt GOV} TLD, with many of its subdomains supporting DNSSEC; hence, we mostly focus on this domain and its subdomains.% to explore properties we may expect in DNSSEC deployments. 
%
%One reason for the slower-then-desired adoption of DNSSEC, may be a belief that current DNS (without cryptography), is secure against the (common) off-path, spoofing-only attacker, and DNSSEC is only required against the (stronger, less common) MitM attacker. 
%% Recently, the deployment rate of DNSSEC increased significantly, when the . Since then, many top level domains (TLD) adopted DNSSEC and serve signed resource records.
%We show that in fact, current {\em DNS is still often vulnerable to off-path attackers}. Specifically, we present efficient and practical off-path poisoning attacks, against many current DNS domains using prominent resolvers. %, which do not (properly) deploy or validate DNSSEC (or other appropriate security mechanism).  
%These attacks completely bypass currently widely-deployed non-cryptographic defenses, such as DNS identifier field, source port randomisation \cite{rfc5452}, 0x20 encoding \cite{DagonAVJL08}, and more. 



\ignore{
\begin{table}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline 
Attacks & \multicolumn{4}{c|}{Poisoning}  &  \multicolumn{2}{c|}{NS-pinning} \\ \cline{2-7}
       & \multicolumn{2}{c|}{Existing } & \multicolumn{2}{c|}{NX-child} & Block & Poison \\ \cline{2-5}
   & NX         & Real & NX & Real  & & \\ \cline{1-2}
Requirements   &           &   &   &    & & \\ \hline \hline
$\begin{array}{ll} \textrm{PR or}\\ \textrm {NSEC} \end{array}$ & $\surd$ & $\surd$ & & & & \\ \hline
Miss-auth & & $\surd$ & & $\surd$ & & \\ \hline 
%$\begin{array}{ll} \textrm{NoNX or}\\ \textrm {IgnoreNX} \end{array}$ & $\surd$ & & $\surd$  & & & \\ \hline
Nx-Auth & $\surd$ & & $\surd$ & & & \\ \hline
Opt-out & & & $\surd$ & $\surd$ & & \\ \hline
NX-Frag & & & & & $\surd$ & $\surd$ \\ \hline
Glue & & & & & $\surd$ & $\surd$ \\ \hline
RFC & & & & & $\surd$ & $\surd$ \\ \hline
\end{tabular}
\caption{Our attacks and requirements}
\label{attacks:table}
\end{table}
}
%On the other hand, ironically, it is exactly the use of DNSSEC which is the main reason for use of EDNS0 for sending long DNS responses, often causing IP fragmentation, which is essential to our attack (on the implementing domain or subdomains). Indeed, our attacks are mostly relevant when a top-level domain implements DNSSEC but subdomains do not deploy DNSSEC (correctly); 


%if  resolvers and clients do not (properly) validate DNSSEC responses, e.g., due to lack of deployment or interoperability concerns, or when no chain of trust can be established to the DNSSEC-enabled zone, in which case the resolver falls back to non-validating mode. 

%In fact, when DNSSEC failures are ignored, the use of DNSSEC resource records (RRs) {\em increase} the vulnerability, since the DNS responses are long (and often/easily fragmented). 

%Furthermore, when a DNSSEC enabled domain uses NSEC3 opt-out records (see section 6 of \cite{rfc5155}), then an {\em off-path} attacker can create a fake response containing a fake (non-existent) sub-domain. The MitM variant of this attack was presented by \cite{bau2010security}, who showed how it allows efficient interception of clients' HTTP cookies. %; however, to add the fake subdomain, they user a man-in-the-middle attacker. We show that this attack can be accomplished even by merely an off-path, spoofing adversary.

%We also observe that fragmented DNS responses, in particular from DNSSEC protected domains, are vulnerable to effective, practical blocking of DNS responses, preventing resolvers from receiving responses from the domains. %This can be abused as part of DoS attack, or to prevent responses to security-critical requests, e.g., to cause failure of automated update services for software. 

%DNSSEC is a standard mechanism designed to protect the DNS resolvers against DNS cache poisoning attacks by man-in-the-middle (MitM) and weaker adversaries \cite{rfc4035}. DNSSEC was conceived more than 15 years ago, and has been in `incremental design and development' since then, to adjust the initial standard to real life systems, in order to facilitate deployment and to patch vulnerabilities; 


%We present practical poisoning and DoS attacks on DNS resolvers, by off-path spoofing adversaries. 
%All of our attacks sidestep the protection offered by widely-deployed defenses such as source port randomisation and 0x20 encoding. Furthermore, the DoS attacks are effective even against domains and resolvers which deploy cryptographic protection such as DNSSEC. 
%


\subsubsection*{Related Work.} Our work builds upon previous disclosures of vulnerabilities due to the design or implementations of the fragmentation mechanism; we next mention few of the most relevant. Zalewski \cite{Zalewski} suggested that it may be possible to spoof a non-first fragment of a (fragmented) TCP packet. However, using such non-first-fragment injections to TCP packets seems challenging. Furthermore, currently almost all TCP implementations use  path MTU discovery  \cite{rfc1191,rfc4821} and avoid fragmentation. 

Several vulnerabilities related to IP fragmentation, and specifically to predictable fragment identifiers (IP-ID) values, are covered in \cite{gont11identification,rfc6274}. %In particular, \cite{gont11identification} discusses vulnerabilities related to the use of predictable fragment identifiers (IP-ID) values. 
Later, predictable IP-ID values were shown \cite{GH:WOOT11} to allow interception and injection of fragments, as well as dropping of fragmented packets. While for our purposes, a simple, randomised modification of fragments suffices, we modify the technique from \cite{GH:WOOT11} to improve the efficiency of the attack in some scenarios; details within. %We apply this to DNS responses, allowing an off-path spoofing attacker to perform DNS poisoning and responses blocking attacks. 
%Gilad and Herzberg extended these results, showing that predictable IP-ID values can allow interception and injection of fragments, as well as dropping of fragmented packets; our attacks build on their results, showing how to apply them to DNS poisoning and DoS attacks. 

%In the original design and specifications of DNS, responses over UDP were restricted to 576 bytes, hence were almost never fragmented. Longer responses are sent over TCP (which usually uses path MTU discovery instead of fragmentation). However, currently, most DNS servers support the {\sf opt} resource record~\cite{rfc2671}, usually referred to as {\em EDNS} (Extensions mechanisms for DNS); more details on EDNS appear in Appendix, Section~\ref{sc:edns}. EDNS allows use of UDP also for long responses. The motivation for EDNS is the fact that using TCP for DNS queries involves significant overhead, in particular, the name servers need to maintain buffers for the duration of the connection; indeed, DNSSEC, which uses long RRs and responses, was an important motivation for EDNS, and DNSSEC queries must use EDNS. 
%Other long resource records which use EDNS include CERT (certificate) resource records, NAPTR and some TXT (textual) resource records.

%Denial of service is possible, whenever DNS responses are fragmented, using the techniques of \cite{GH:WOOT11}. We further show that in common scenarios, poisoning is also possible, and often require modest attacker capabilities and resources. 

\ignore{
\subsubsection*{Attack Requirements.} The feasibility of poisoning, and the required attacker capabilities and resources, depend on 
several factors (summarised in Table~\ref{attacks:table}), motivating different attack variants. 
% of the attack (presented within - and others yet to be found). 
The factors include:\\
%\begin{description}
\indent {\sc Permissive Resolver:} a resolver that signals support of DNSSEC in queries (DO bit), but does not discard a DNS response that fails DNSSEC validation. Currently, many resolvers support such permissive mode, due to interoperability concerns.\\
\indent {\sc Island:} a child DNS  zone that implements DNSSEC, but is not properly signed by the parent zone. \\
% & $\surd$ & $\surd$ & & & \\ \hline
\indent {\sc Authority Section:} the second fragment of the response contains complete record(s) from the Authority section (e.g., NS record).\\ %& $\surd$ &  &  $\surd$ & & \\ \hline 
\indent {\sc Additional Section:} the second fragment of the response contains complete record(s) from the Additional section (e.g., A record).\\% &  & $\surd$ & &    & $\surd$\\ \hline
%$\begin{array}{ll} \textrm{NoNX or}\\ \textrm {IgnoreNX} \end{array}$ & $\surd$ & & $\surd$  & & & \\ \hline
\indent {\sc Any Size Fragment:} any fragmentation, even of a single byte, suffices.\\ %& & &  &   $\surd$ & \\ \hline
\indent {\sc NSEC3 opt-out:} a zone that uses the NSEC3 opt-out option, namely, does not provide `proof of non-existance' for child zones which do not deploy DNSSEC (or, that the zone is not aware of their use of DNSSEC). This allows creation of fake child zones.\\ %& & & $\surd$ &  & \\ \hline
%5. NXD-Frag & & & & & $\surd$ & $\surd$ \\ \hline
\indent {\sc RFC 4697:} resolver that follows recommendations in RFC4697, to avoid - for a fixed interval - unresponsive name servers, i.e., from which there were few lost DNS responses.\\ %& & & &  $\surd$ & $\surd$ \\ \hline
}
%\item[DNSSEC.] %DNSSEC is main motivation for long DNS responses which use EDNS and get fragmented, facilitating the attacks; on the other hand, w
%When DNSSEC is properly deployed by resolvers, then poisoning of domains which properly use DNSSEC appears infeasible \cite{bau2010security}; if NSEC3 opt-out is avoided and all sub-domains are protected, then poisoning is prevented. However, blocking of DNS responses (for DoS) is still feasible. Furthermore, {\em partial or incorrect deployment of DNSSEC may allow poisoning}. %In particular, our poisoning techniques work in any of the following cases: (1) when a resolver does not deploy DNSSEC or ignores validation failures, (2) when a resolver does not have the DNSKEY of the target zone and cannot establish a chain of trust to the `island of security', and (3) when a domain is not protected by DNSSEC (yet relevant responses are fragmented, possibly, from a higher-level domain). 
%
%\item[Contents of fragments.] To cause loss of DNS responses, for server pinning, any amount of fragmentation suffices. Our other poisoning attacks mostly require some resource records in the second fragment of the response. Depending on the trust policy of the resolver, it may be  necessary to have a resource record from the `authority' or even `answer' part of the response, see \cite{son2010hitchhiker}. While DNSSEC deployment is still only beginning, there are already many such domains; e.g., as Fig. \ref{fig:lengths-of-gov} shows, the responses of more than a half of the domains in {\tt GOV} are of size larger than 1500 bytes, when queried for an {\tt ANY} RR, which can be generated by zombies; and a significant fraction also have {\tt non-existing domain} responses of length over 1500 bytes, which can be generated by a puppet or by opening an email connection to a mail server using the resolver. Of course, in some networks (links), the MTU is less than 1500 bytes. %; furthermore, we present some techniques that can cause fragmentation of responses, even when responses do not exceed the MTU of 1500 bytes. 
%Note that some top level domains, notably {\tt gov, edu} and {\tt com}, are rarely fragmented, since they use TCP rather than UDP to send long responses; the motivation is apparently interoperability\footnote{Fragments are often blocked, \cite{nominet:study}, rendering the clients with no DNS functionality.}, as using TCP has considerable overhead, and would hopefully only be an interim solution. 
%Note that currently most domains use a small number of keys or short (and thus weak) cryptography, e.g., 1024 bit RSA keys. When stronger cryptography (or more keys) is used the DNS response size will significantly increase, exacerbating the vulnerability.
\ignore{
\item[Fragment ID.] Our attacks are most efficient if attacker can predict the IP-ID value in the IP header of the response packet fragments. As shown in \cite{GH:WOOT11}, these values are  predictable for the common case where the IP-ID is globally-incrementing (e.g., Windows) or per-destination incrementing (e.g., Linux). We found that some name servers are neither globally-incrementing nor per-destination incrementing, yet, their IP-ID values were also easily predictable. We did not find name servers using highly-unpredictable IP-ID values, however, such may exist; yet, our poisoning attacks would still be effective, in particular in light of the ability to use multiple matching queries, using the `birthday paradox'; see subsection \ref{sc:bd}. 
}
\subsubsection*{Attacker Capabilities.} %The attacker can use different mechanisms to cause the resolver to generate the request, resulting in fragmented response, amenable to poisoning. 
The required attacker capabilities include an arbitrary off-path, spoofing-only adversary, that controls a `puppet', i.e., malicious (but sandboxed) script which can query the resolver; see Figure~\ref{fig:simple:attack:scenario}.
%ultimately to a 
%user-mode\footnote{Note that assuming such user-mode zombie, while a significant assumption, is still a relatively weak assumption; in particular, esp. with newer operating systems, most malware operates only as user-level zombie, and cannot send spoofed packets or perform sniffing, as required, e.g., for ARP poisoning.} `zombie', i.e., machine running attacker's malware. 
%%Notice that our spoofing-only attacks, require specific (but common) network scenarios, specifically, either an open resolver, or a resolver used by an incoming mail server (MTA) which applies SPF or DKIM validation \cite{journals/H:DNS:based:ea}. 
%See Figure \ref{fig:simple:attack:scenario}.
%\end{description} 
 


%Note that some name servers, e.g., of GOV, EDU and COM top-level domains, send DNS responses larger than 1500 bytes over TCP rather than over UDP. This is probably due to the fact that some firewalls may block fragmented traffic. This foils our attacks; however, due to the high at a high overhead to the name server (and modest additional overhead to the resolver and to the network). Indeed, this is one possible way to prevent our attacks. However, due to the significant overhead, we recommend this solution only for the near term, as a stop-gap measure. We provide more details on recommended defenses in Section \ref{s:defenses}. 

%\subsection{Attacker Capabilities}
%As in other works on DNS poisoning, we assume an off-path, spoofing adversary that can send packets with forged source IP address, but cannot observe or modify the traffic.
%In addition, our attack require the ability to send DNS requests to the victim resolver. 
% 
%The mere assumption of an off-path, spoofing attacker suffices for some of our DNS cache poisoning attacks. Spoofer-only attacks can be launched when domain has MX or TXT records that result in sufficiently large responses, we show DNS cache poisoning via mail transfer agent (MTA) (Section~\ref{s:MTA}). Spoofer-only attacks also hold against open recursive resolvers (Section~\ref{s:open-resolver}), where the attacker can query the resolver, which it wishes to poison, with arbitrary DNS requests. 

\begin{figure}[!ht]
\begin{center}
%\fbox{
    \epsfig{scale=0.4,file=attack-scenario-puppet3}
%     }
\end{center}
\caption{\footnotesize{Simplified network topology and attacker capabilities. The spoofing attacker uses a puppet to invoke the query.}}
 \label{fig:simple:attack:scenario}
\end{figure}

%To poison resolvers which do not provide open recursive service, i.e., only serve clients on their LAN, or when exploiting mail transfer agents is not possible, e.g., no mail server, our attacks require an insider which can query the DNS resolver.
%An insider can be a malicious script confined in a browser or a malicious software (malware) with `user level' privileges, i.e., the malware does not require spoofing capabilities and cannot eavesdrop or inject spoofed packets. The attacker (controlling a `puppet') and abstract network topology are depicted in Figure~\ref{fig:simple:attack:scenario}; the spoofer lures a client to visit its web page, and the client becomes a `puppet', i.e., used by the attacker to issue DNS requests to the resolver.
%(Section~\ref{s:simple-attack})
\ignore{
\subsection{Example of the attack} %Poisoning/Blocking Fragmented\\DNS Responses}
%The basic idea of the fragmentation-based DNS poisoning and blocking attacks, is to modify a fragmented DNS response packet. 
%To modify a fragmented packet, similarly to \cite{GH:WOOT11} which showed how to exploit fragmentation for denial of service, we send a forged second (or/and subsequent) fragment(s) to the resolver, so that it is reassembled with the legitimate fragment(s) once they arrive. 
%There are several challenges involved, including the fact, that most DNS responses are too short to be fragmented, and furthermore, even a fragmented packet may not allow easy poisoning; see following sections for details. Here, in the introduction, we  explain the main ideas behind the fragmentation-based DNS attacks. 

%, by discussing a (simple) example, and then presenting the three phases of the attack. 
To illustrate the main ideas of the fragmentation-based poisoning attacks, we %first
discuss one simple variant, where we forge the second fragment of a DNSSEC response. The reason we use a DNSSEC response, is to obtain a sufficiently large response, that would be fragmented. We send a forged second fragment, containing fake resource record(s). This forged second fragment stays in the defragmentation cache until the authentic first fragment of the response arrives, and then, the defragmentation process combines it with the authentic first fragment, resulting in a seemingly-valid response. The poisoning attack succeeds if the resolver accepts this response as valid and adds the fake RRs to its cache.

The annotated screen caption presenting a variant of our attack is in Fig. \ref{fig:forged:resp:info}. The figure shows a poisoning of DNSSEC enabled response against resolvers that do not perform strict DNSSEC validation. The first line (122) contains the `forged second fragment'; this fragment is kept in the defragmentation cache of the resolver, waiting for a matching first fragment (i.e., with the same set of {\tt (source IP=199.249.112.1, dest IP=132.70.6.202, fragment ID=7c6e, protocol=UDP)}). 

In the next line (133), we find the DNS query sent to the name server. This is a DNSKEY query sent to the (name server of the) ORG top-level domain. Note that the DNSKEY query is issued automatically by DNSSEC-complying resolvers, e.g., as part of handling other queries; an attacker may also be able to cause a resolver, which does not support DNSSEC, to issue such a query, by sending an appropriate request to the resolver. 

Next line (134) is the first fragment of authentic response to the query, sent by the name server of ORG (at IP 199.249.112.1). This response matches the fake second fragment already in the defragmentation cache, hence it appears as a complete DNS response packet. The contents of this packet are described in the lower panes; in particular, see the two forged resource records in the additional section, which contain incorrect (adversarial) IP addresses for two of the name servers  of the ORG domain. In many cases, these records would be entered into the cache of the resolver (we discuss the conditions for this later on). 

Finally, notice that the authentic second fragment, received in line 135, has no matching first fragment (since the one received was already reassembled with the spoofed second fragment). Hence, it is entered into the defragmentation cache, where it is likely to remain until discarded (typically, after maximal lifetime of about 30 seconds). 



\subsection{Attack phases} 
In the simple attack example above, we focused on the {\em response phase} of the attack. The response phase is the main and final phase of the attack: the delivery of the forged fragment, which causes the resolver to handle a response packet containing fake resource records (and often enter the poisoned response to the cache). Notice, that this happens only after the resolver sends the corresponding query, in the {\em query phase}. 

Furthermore, often, the attack may involve an even earlier (optional) phase, the {\em preprocessing phase}. The preprocessing phase ensures appropriate conditions for the query and response phases, by optionally performing one or both of the following two tasks. The first task is to find the expected value of the fragment IP-ID field;  we can use the same techniques as in \cite{GH:WOOT11}. The second task is to cause fragmentation (even for relatively short responses), using fake ICMP `fragmentation required' packets. 

We illustrate all three phases of the attack in Fig. \ref{fig:flow}. 
}
%%All our attacks exploit {\em IP fragmentation}, by sending spoofed fragments, facilitating  to combine with the legitimate response. 
%Fragmentation is a side effect of (long) DNS responses. 
%Such long UDP responses are possible for DNS, when using . 
%The use of EDNS, to support long responses, is very common, since the essential for DNSSEC, 

%Sufficiently-long DNS responses are quite common. Ironically, DNSSEC is one cause for such long DNS responses; other causes for long DNS responses include CERT and some TXT resource records.
%Attackers may use ICMP, to reduce the response-length requirement, i.e., cause fragmentation even for responses shorter than the path MTUfor shorter responses; this works foin , with the required path MTU, on the DNS server, using ICMP. 


%We present a weakness allowing DNS poisoning, pertaining to Domain Name System (DNS) %\footnote{We discuss the DNS poisoning threat in full version of the paper.} 
%{\sf opt} resource record~\cite{rfc2671}, usually referred to as {\em EDNS} (Extensions mechanisms for DNS). 
 




%Briefly, EDNS allows to serve long DNS responses over UDP. Most notable use of EDNS RR is to signal support of DNSSEC and to transfer long DNSSEC responses. In particular, the client indicates the EDNS buffer size (default is 4096 byte) and the sender limits the response to that size. Since DNSSEC enabled responses contain keys and signatures, the responses often result in fragmentation. 

%We validated our attacks on two caching DNS resolvers, both supporting DNSSEC: {\em Bind} and {\em Unbound}. The resolver queried real TLD DNS servers on the Internet. Another machine acted as an off-path spoofing adversary, and sent fake responses to the resolver. 
%%In some attacks the spoofer was connected via a switch to the same LAN as the resolver, while in other scenarios the spoofer was on another network, and the resolver was behind a NAT or a firewall.
%Both resolvers were vulnerable, but there were significant differences; details within. 

 

%In the course of our attacks we poisoned the resolvers' entries for several prominent top level domains (TLDs), including: ORG, INFO, BIZ, US, SE, and others. Our attack did not work against the name servers which serve long responses over TCP, e.g., COM, GOV, EDU TLDs, however, the RRs for prominent subdomains of those TLDs are susceptible to attacks, e.g., Verisign.COM, cmu.EDU. Also note that our attack does {\em not} break DNSSEC itself; namely, properly signed records cannot be poisoned, in properly configured resolvers. Note, however, that there may be (many?) resolvers configured to accept records which are supposed to be DNSSEC-signed, but sent without appropriate signature - these may be vulnerable. 





%\subsection{Our contributions}
%
%************** add here!! [or: remove in draft for review] ***********

\subsubsection*{Contributions.}
%We outline our attacks and their requirements in Table~\ref{attacks:table}, and also summarise them below.
\begin{description}
	\item [Incremental DNSSEC Deployment is Vulnerable] We show that incremental deployment of DNSSEC is risky, and exposes resolvers to cache poisoning attacks. We present techniques which allow efficient and effective Kaminsky-style~\cite{kaminsky:dns} cache poisoning attacks, using off-path spoofing adversaries. Our techniques (exploiting fragmentation) allow to circumvent the entropy (randomisation of query, source port and IP) in DNS responses, as those entropy fields remain in the first fragment. This exact technique of circumventing the entropy fields allows us to revive the Kaminsky attack, and to replace the authentic records in a DNS response with spoofed records. 
	\item [Subdomain Injection] We show that an off-path attacker can perform the attack that was believed to be feasible for MitM.
	\item [Unsigned Delegation] We suggest attacks exploiting unsigned NS and A delegation records, breaching privacy and anonymity, and inflicting denial/degradation of service.
	\item [Name Server (NS) Blocking] We introduce the name server blocking technique, which allows an attacker to force the resolver to stop using a particular name server, and eventually, to query a name server of attacker's choice, e.g., a compromised name server, when resolvers strictly follow RFC 4697 \cite{rfc4697}. 
\end{description}
We performed an experimental evaluation of our attacks against standard resolver software and issuing queries to real TLD name servers, such as {\sf org}, and against the name server of the domain of our university, i.e., {\sf sec.cs.biu.ac.il}.
\subsubsection*{Organisation.}
In Section~\ref{sc:requirements} we outline the assumptions which are required for our attacks and in Section~\ref{s:open-resolver} we provide the basic mechanisms for our attacks. Then, in Section~\ref{sc:ip}, we show techniques for name server blocking, and in Section~\ref{sc:poisoning} we present the poisoning attacks. We then conclude and propose defenses in Section~\ref{s:defenses}. % the next section, we present the different variants of the response phase of the attack. Then, in Section \ref{sc:query}, we discuss the query phase, and in Section \ref{sc:pre}, the preprocessing phase. 
% In Section~\ref{s:open-resolver} we show DNS cache poisoning attacks which exploit fragmentation to forge the second (and/or subsequent fragments) of a DNS response. However, these attacks require that the second fragment contains at least one full DNS record. When this assumption does not hold, we suggest extensions, in Section~\ref{first:frag:attack}, and show how the attacker can intercept the first fragment, and poison the `whole' DNS response, or launch denial of service attacks when interception is not feasible. In Section~\ref{sc:query} we consider the ways in which attacker can trigger a DNS request that would produce the required response, and how to evade the caching of the resolver. In Section~\ref{sc:pre}, we show that the attacker can employ different techniques during the `preprocessing phase' to enforce fragmentation of DNS responses, and to make the guessing of the IP-ID more efficient. 
%Finally in Appendix we describe the problems in DNSSEC deployment (Section \ref{sc:permissive}) and outline conditions required for resolvers to cache poisoned DNS records (Section~\ref{sc:conditions}).

\ignore{
Two variants: 
A. Attack on long responses: DNSKEY responses, where attacker controls a subdomain of a TLD, and the expriration is sufficiently short.
Then improving the ID and improving the caching, and then improving: long responses are not required.

B. NSEC3 responses (allow to avoid caching), if the responses are sufficiently large or MTU sufficiently small.
C. When the second fragment does not allow us to inject the fake fragment - use attack that replaces the first fragment. 


Discovering the IDs or sending all possible IDs.
Discovering the ID using the puppet, based on the times.
2. 

Free BSD and Microsoft use predictable IP-ID.
}
\ignore{
impact on: certificates in TXT...
Poisoning the root
}
\ignore{
\subsection{DNS Poisoning}
Correct and efficient functionality of DNS is important for the functionality of the Internet. In the recent years, the most significant attack on the Domain Name System (DNS) is {\em DNS poisoning}, where the attacker tries to provide incorrect mappings to DNS queries. DNS poisoning can facilitate many other attacks, such as injection of malware, phishing, website hijacking/defacing and denial of service, see~\cite{Kaminsky08,VU800113}. 

The most effective DNS poisoning method is to send a fake (spoofed) response to a DNS request. DNS request contains an identifier field which should be returned by the domain name server in each response, however, this field is only 16-bits long, hence attacker can succeed by sending a reasonable number of responses. Furthermore, some DNS implementations use predictable identifiers (sequential, or using a weak pseudorandom generator); for example, in~\cite{Klein07:Bind9Poisoning}, Klein shows how to predict the identifier for the then-current version of Bind 9, a widely-used DNS server, and how this can be exploited for highly-efficient DNS poisoning by a spoofing attacker. 

Bernstein suggested to improve DNS's defense against spoofed responses by sending the request from a {\em random port}, which can add a significant amount of entropy\footnote{The exact amount of entropy added depends on the number of available ports, which may be below $2^{16}$.}.
While this vulnerability has been known since 2002 (and fixed in some DNS servers), see \cite{Bernstein:DNS}, many implementations ignored it till Kaminsky recently showed, \cite{Kaminsky08,VU800113}, an attack with two critical improvements.
The first improvement was to control the time at which the resolver sends queries (to which the attacker wishes to respond), by sending to the resolver queries for a non-existing host name, e.g., with a random or sequential prefix of the domain name. Each time the attacker may send multiple DNS requests for the same host name to maximise the probability of a match of the ID and port selected by the resolver with one of the responses which the attacker will send (taking advantage of the `birthday paradox'). 
Notice that if the attack for a given host name (prefix) fails, the attacker simply uses a different prefix.  
Kaminsky's second improvement of the poisoning attack was to add, in the spoofed responses sent to the resolver, a type {\sf NS} DNS record (specifying a new name for the domain name server) and/or a type {\sf A} `glue' DNS record (specifying the IP address of that domain's name server). These records poison the resolver's entries for the victim name server. Hence, if the attack succeeds once (for one record), the adversary controls the entire name space of the victim. 

Using these two improvements attackers can often poison the DNS entry for the victim domain, when the resolver is using a fixed port, within few seconds! This allows devastating attacks on many Internet applications.
}



==> poisoning.tex <==
\section{DNS Response Poisoning}\label{sc:poisoning}
The main idea behind our DNS cache poisoning attacks is to apply Second-fragment Overwriting technique to change the content of a DNS response by replacing authentic resource records (RRs) with spoofed A or NS RRs either for the existing domain or for a new subdomain. Specifically, the off-path attacker triggers a DNS request to some victim domain, e.g., using a puppet (malicious script confined in a browser), and then spoofs the second fragment. Depending on the section (of the DNS response) which the second fragment contains, i.e., {\tt authority} or {\tt additional}, the attacker replaces authentic records with his fake records\footnote{The attacker can also replace the RRs in the {\tt answer} section, e.g., if it can issue DNS requests for ANY type RR, and if the DNSSEC is either incorrectly, or not at all, deployed.}. 

The main difference between the attacks is related to the two intertwined issues: (1) frequency at which the attack can be repeated, and (2) the queries which the attacker can request. Both these issues depend on the freedom of the attacker over the (suitable) queries which it can request.

\paragraph{NXDOMAIN or No-Data Responses.} To evade caching of the resolver the attacker can issue DNS requests for `non-existing domain names', i.e., responses containing an RCODE with name error, or responses indicating that the domain name exists but with a different type, i.e., with `no data no error' responses. Such responses exist in {\em every} domain. We found that domains that use NSEC3 (which is currently the majority of the domains) to indicate nxdomain (and no data) responses, to be most suitable for our attacks as those responses get fragmented in the {\tt authority} section, such that the second fragment contains at least one complete RR (not including the EDNS RR). This technique is similar to Kamisky attack, as it allows the attacker to repeat the attack as frequently as required, by selecting a different random name (prepended to the real domain name) in each query.
However, nxdomain responses may not always get fragmented, e.g., if the zone does not use NSEC3.

\paragraph{`Existing Domain' Responses.} If the attacker triggers the attack with queries for existing domain names (with a non-zero TTL) that get fragmented, e.g., responses to DNSKEY, then it can trigger the attack only if the record is not in cache. If the attack fails the first time, it has to wait till the record expires from cache, i.e., the TTL reaches 0 or sinature expires. %; we show an attack exploiting a response to a DNSKEY RR.

Records with zero TTL, e.g., used for CDN networks, can be requested repeatedly, thus allowing to launch the attack as frequently as required, since they are not cached. Such DNS responses with (zero TTL) records in the {\tt answer} section also contain (among others) NS and A records (in {\tt authority} and {\tt additional} sections respectively) with a cache-able TTL, which the attacker can replace. However, the zero TTL records may not exist in every domain, and in particular, may not exist in a domain which the attacker wishes to poison.

Thus the typically query choice of the attacker is between `nxdomain/no-data' or `exiting domain' (with a non-zero TTL).

%e.g%., when can the attack be launched again if it failed the first time (say due to failed checksum calculation), 

\paragraph{Poisoning the Cache.} 
Inserting spoofed records into the cache is not straight forward, and merely changing the records in a DNS response will not necessarily result in resolver accepting and (then) caching them. In particular, the forged DNS response must comply with the caching (and other) conditions which the resolvers impose on DNS responses: the forged packet $p'$ must be a valid DNS response; the `poisonous' resource record $r'$ must be valid for the specific response and section of the response; and the resolver must cache $r'$. %We elaborate on each of these conditions in Appendix~\ref{sc:conditions}. 

The choice of forged DNS records, which we apply when modifying the DNS response, and semantics and values of each field in a DNS record, essentially follow the known rules for DNS cache poisoning and were investigated and studied (most notably) by Kaminsky~\cite{kaminsky:dns} and Son and Shmatikov~\cite{son2010hitchhiker}, and by Bau and Mitchell~\cite{bau2010security} for DNSSEC enabled DNS responses.

\subsection{Domain Hijacking} \label{sc:DomHij}

Domain hijacking can be performed when the \Rdnssec\ requirement is satisfied in tandem with \Rpz, i.e., either the resolver is permissive or zone is an island of security and there is at least one RR in the second fragment. In this case the attacker can replace the RR(s) in the authentic second fragment of a DNS response with (spoofed) NS or A  RR(s) pointing at his name server; the TTL in those spoofed RRs has to match the TTL of the other RRs in that RRset. 

Note that our domain hijacking techniques (below) trivially apply to (fragmented) DNS responses which are not protected with DNSSEC, we show such attack, exploiting queries for TXT RRs and the corresponding responses that get fragmented in full paper (the attack course is essentially similar to the attacks presented next).

%This attack can have two impacts: (1) If the resolver does not perform strict DNSSEC validation (or if the domain were an island of security), then the attacker can hijack the the name servers for {\tt org} domain hijaking all of {\tt org's} subdomains. The impact of this attack is effectively equivalent to the Kaminsky poisoning attack. Yet it is practical as it circumvents all the defenses against Kaminsky attack, e.g., source port randomisation. (2) In contrast, if the resolver performs strict validation of the DNSSEC responses, then the attacker can perform `server-pinning' by applying the technique in Section~\ref{sc:ip} and blocking the rest of the name servers of {\tt org}.%; this can be useful, e.g., for traffic analysis or covert communication, when DNSSEC is correctly deployed.

We tested the domain hijacking attack in two scenarios (as elaborated above): (1) nxdomain/no-data and (2) existing domain. The `nxdomain/no-data' (NSEC33) response is often fragmented in the {\tt authority} section, and the {\tt additional} section contains an\footnote{This is not a requirement, and according to \cite{rfc2308} an A RR can appear in the {\tt additional} section too. In this case, the attacker simply replaces the A RR (instead of NS).} EDNS RR. This allows replacing the {\tt authority} records in the second fragment with fake NS RRs; we show this attack in Section~\ref{ssc:ns} replacing an NSEC3 record with a spoofed NS record in the {\tt authority} section in response to a request for some non-exiting domain within {\sf sec.cs.biu.ac.il}, i.e., the (DNSSEC-enabled) domain of the security group of the computer science department within our university.. The `existing domain' response, e.g., DNSKEY or TXT, is also often fragmented. Such responses typically contain records in the {\tt additional} section too, and allow changing the IP of name server with IP of the attacker. We show this attack in Section~\ref{ssc:a}.
%(1) replacing the A record in the {\tt additional} section against the {\sf org} domain in response to a DNSKEY DNS request; as well as (2) 

\subsubsection{Injecting NS RR to NSEC3 Response}\label{ssc:ns}
Typically, responses of type `non-existing domain (nxdomain) name error' or `no data no error', in domains that support NSEC3, %, contain one RR, the EDNS, in the {\tt additional} section, and the rest of the RRs, i.e., SOA, NSEC3, in the {\tt authority} section. Such NSEC3 responses are typically 
are of size between 1700 to 2000 bytes on average, and when fragmented, at least one record from the authority section appears in the second fragment. This allows the attacker to replace the authentic NSEC3 or RRSIG RR(s) with a NS RR for a new name server; Figure~\ref{fig:nsec3}. If the response does not contain any other NS RRs then the attacker can set an arbitrary high TTL, e.g., 6 days, to ensure that his RR stays in cache even when the authentic NS RRs for that domain expire.
 \begin{figure}[!ht]
\begin{center}
%\fbox{
    \epsfig{scale=0.27,file=nxdomain}
%     }
\end{center}
\caption{\footnotesize{Poisoning an nxdomain (or no data) response, by replacing the NSEC3 RR with an NS RR.}}
\label{fig:nsec3}
\end{figure}
The attacker triggers a DNS request (via a puppet) and synchronises (steps 1 and 2, Figure~\ref{fig:nsec3}). Then (step 3) the attacker sends a spoofed second fragment containing an NS RR for domain {\sf sec.cs.biu.ac.il}. This spoofed fragment is combined with the authetic first fragment (step 3) and enters the cache; the authentic second fragment is discarded after a timeout (step 5). Note that the attacker can provide any arbitrary NS RR, in particular, one that is not in the same domain as the victim; in this attack we spoofed the response with name for a new NS RR, i.e., {\sf {\bf ams}.sec.cs.biu.ac.il}, in our domain, i.e., {\sf sec.cs.biu.ac.il}, for testing purposes to observe that the subsequent queries of the resolver to domain {\sf sec.cs.biu.ac.il} are sent to {\sf ams.sec.cs.biu.ac.il} and responses get cached. To find the IP of the new NS the resolver initiates a request for the A RR, and receives and caches the IP supplied by the attacker (who controls that name server). 

The wireshark capture of the resulting poisoned DNS response is in Figure~\ref{fig:nsec3:biu:spoofed}. The authentic fragment contained part of the RRSIG and two complete records, i.e., NSEC3 and a corresponding RRSIG. The spoofed fragment contained the authentic part of the RRSIG, spanning the first and second fragments, and two fake NS records which replaced the authentic NSEC3 and RRSIG. Note that since the RRSIG (as well as NSEC3) are much larger than NS RRs, the attacker has to pad the packet (with zeros) to the required length; the checksum is adjusted in the padded area after the EDNS RR.
\begin{figure*}[!ht]
\begin{center}
%\fbox{
    \epsfig{scale=0.70,file=nsec3-biu}
%     }
\end{center}
\caption{\footnotesize{Poisoning an nxdomain (or no data) response for domain {\sf sec.cs.biu.ac.il}, by replacing the NSEC3 RR with an NS RR.}}
\label{fig:nsec3:biu:spoofed}
\end{figure*}
For a comparison, see the authentic DNS response in Figure~\ref{fig:nsec3:biu:auth}.
\begin{figure}[!ht]
\begin{center}
%\fbox{
    \epsfig{scale=0.60,file=nsec3-biu-auth}
%     }
\end{center}
\caption{\footnotesize{An authentic nxdomain response for domain {\sf sec.cs.biu.ac.il}.}}
\label{fig:nsec3:biu:auth}
\end{figure}
\subsubsection{Injecting A RR to DNSKEY Response}\label{ssc:a}
When the second fragment contains at least one complete record (excluding the EDNS RR) in the {\tt additional} section, the attacker can replace the IP address in the fragment with a spoofed IP. In this attack we spoof the IP for the name server of {\sf org} domain, in a DNS response for a DNSKEY of {\sf org} domain.

In Figure~\ref{fig:org:attack} the resolver issues a DNS request for the DNSKEY of {\sf org}; this is an indirect way to trigger a query, i.e., the resolver asks for the DNSKEY of some domain automatically, when the DNSKEY expires from cache, or when it needs to validate records for that domain, e.g., to be able to validate an A record or a non-existing domain (NSEC3) record; an attacker may also be able to cause a resolver, which does not support DNSSEC, to issue such a query, by sending an appropriate request to the resolver. This query type is useful if the response to an nxdomain query is not fragmented.
\begin{figure}[!ht]
\begin{center}
%\fbox{
    \epsfig{scale=0.33,file=org-ns}
  %   }
\end{center}
\caption{\footnotesize{DNS poisoning attack of name server IP of {\sf org} domain. The resolver issues a query for a DNSKEY (e.g., when it expires from cache, 15 minutes for {\sf org}), and the spoofer sends a poisoned second fragment containing the forged entries of {\sf org}. The query for DNSKEY of {\sf org} can also be triggered indirectly by issuing a query for non-existing (or for some other) domain within {\sf org}.}}
 \label{fig:org:attack}
\end{figure}

The annotated screen caption of the attack in Figure~\ref{fig:org:attack} is illustrated in Figure~\ref{fig:forged:resp:info}, presents the outcome of the attack. The first line (122) contains the `forged second fragment'; this fragment is kept in the defragmentation cache of the resolver, waiting for a matching first fragment (i.e., with the same set of {\tt (source IP=199.249.112.1, dest IP=132.70.6.202, fragment ID=7c6e, protocol=UDP)}). 
In the next line (133), the resolver sends the DNS query to the name server. 
%This is a DNSKEY query sent to the (name server of the) {\sf org} top-level domain. Note that the DNSKEY query is issued automatically by DNSSEC-complying resolvers, e.g., as part of handling other queries; an attacker may also be able to cause a resolver, which does not support DNSSEC, to issue such a query, by sending an appropriate request to the resolver. 

Next line (134) is the first fragment of authentic response to the query, sent by the name server of {\sf org} (at IP 199.249.112.1). This response matches the fake second fragment already in the defragmentation cache, hence it appears as a complete DNS response packet. The contents of this packet are described in the lower panes; in particular, see the two forged resource records in the additional section, which contain incorrect (adversarial) IP addresses for two of the name servers  of the {\sf org} domain. %In many cases, these records would be entered into the cache of the resolver (we discuss the conditions for this later on). 

Finally, notice that the authentic second fragment, received in line 135, has no matching first fragment (since the one received was already reassembled with the spoofed second fragment). Hence, it is entered into the defragmentation cache, where it is likely to remain until discarded (typically, after maximal lifetime of about 30 seconds). 
\begin{figure*}[!ht]
\begin{center}
%\fbox{figs
    \epsfig{scale=0.45,file=fake-org-ns}
 %    }
\end{center}
\caption{\footnotesize{A Wireshark capture presenting the DNS packets in a DNS cache poisoning attack exploiting fragmented DNS responses by spoofing the second fragment of the response to the DNSKEY query; messages exhange diagram corresponding to this caption is in Figure~\ref{fig:org:attack}. %This attack works against DNS resolvers that do not perform strict validation of DNSSEC.
%Forged DNS response containing two A RR inserted by the attacker.
}}
\label{fig:forged:resp:info}
\end{figure*}

\subsection{Subdomain Injection} \label{sc:SubInj}
\ignore{
The NS RRset that appears at the zone apex name MUST be signed, but
   the NS RRsets that appear at delegation points (that is, the NS
   RRsets in the parent zone that delegate the name to the child zone's
   name servers) MUST NOT be signed.  Glue address RRsets associated
   with delegations MUST NOT be signed.

   Essentially the same as in Sections \ref{ssc:ns} and \ref{ssc:a}.
}
The delegation records, NS (name server) and A (IP address), located in {\tt authority} and {\tt additional} sections, are not signed, \cite{rfc4035}. This allows the attacker to change the IP address (in the {\tt additional} section) of the name server of some victim domain, to its own address, or to add a new name server (in {\tt authority} section) for the victim domain. Such NS and A records are usually cached and used, for queries to the specified domain; see \cite{son2010hitchhiker}. At this point, the attacker managed to cause queries for the victim subdomain to be sent to a machine controlled by the attacker. %;  

This vulnerability, of redirecting DNSSEC enabled DNS requests to malicious server by a man-in-the-middle, was pointed out by Bernstein~\cite{Bernstein:woot}, yet without a specific application for such an exploit. Bau and Mitchell, \cite{bau2010security}, refute Bernstein's claim of this being a vulnerability, by proving that it does not enable a man-in-the-middle attacker any additional capabilities, and conclude that it does not pose a significant threat. Indeed, not signing the delegation records does not break the design requirements defined for DNSSEC, \cite{rfc4035}. However, it exposes to NS Hijacking (leading to a range of other attacks), Section~\ref{sc:NSInj}, and to subdomain injection (as we discuss next). %Yet, we show that by applying our technique an off-path attacker can `fix' the name server (Section~\ref{sc:fix}) for a victim domain, and as a result perform a range of attacks including: traffic analysis, covert channel attacks, denial of service attacks.


  Resource records in the {\tt answer} section of DNSSEC-enabled domains are signed, hence, if the resolver performs strict validation of DNSSEC, it should not accept unsigned records in the {\tt answer} section. However since the delegation records in the {\tt authority} and {\tt additional} sections are not signed, the attacker can create a new subdomain, e.g., {\sf secure.bank.com} under {\sf bank.com}, by creating an NS record (in the {\tt authority} section) for the new subdomain {\sf secure.bank.com} mapping it to the name server which the attacker controls. % this is modelled in column `New Subbdomain' in Table~\ref{attacks:table}.
This attack is only applicable to DNSSEC protected domains that use NSEC3 opt-out: the attacker may be able to use legitimate NSEC3 responses, e.g., for non-existing sub-domain, or other type responses, e.g., DNSKEY, and turn them into what appears to be a legitimate referral to an unprotected sub-domain; this can be used for phishing attacks. Furthermore, as \cite{bau2010security} show, domains which deploy NSEC3 opt-out records are vulnerable to browser cookie theft by a man-in-the-middle attacker, as they allow the attacker to insert insecure delegations into DNS responses. This is in contrast to the recommendations in \cite{rfc5155} which suggest that NSEC3 opt-out does not pose a significant threat. Bau and Mitchell performed the attack with a man-in-the-middle attacker, using our techniques an {\em off-path} spoofing attacker can perpetrate such attacks, see Figure~\ref{fig:nsec3:biu:spoofed}.

	The attack is similar to the attack in Section~\ref{ssc:ns}, thus to save space, we performed the addition of a new subdomain as part of the name server hijacking attack, see Figure~\ref{fig:nsec3:biu:spoofed}. The record: {\sf www.sec.cs.biu.ac.il} is a new (non-existing) subdomain under {\sf sec.cs.biu.ac.il} and it points at the name server {\sf ams.sec.cs.biu.ac.il} controlled by the attacker. 
%\subsection{Name Server (NS) Injection} \label{sc:NSInj}


\subsection{NS Hijacking}\label{sc:NSInj}
Using `server blocking' the attacker can `fix' the target name server. If the attacker compromised that server then the attack is very damaging. Server fixing can be useful for other attacks too, e.g., to degrade efficiency (if the target server is the slowest), for traffic analysis, e.g., if the attacker has man-in-the-middle capabilities but only on the path to that `fixed' server, but not to other servers for that domain.

Server fixing in tandem with DNS poisoning can allow the attacker to force the resolver to use a malicious name server which the attacker controls, we call this `NS hijacking'. This attack is most relevant when DNSSEC is properly deployed. If the DNSSEC is not deployed correctly, then the attacker can simply hijack the domain. 
The attack is combined of two phases: (1) poisoning the A (or respectively NS) record in the DNS response (by changing the authentic IP to the IP controlled by the attacker), then (2) applying server blocking by ruining responses from all other name servers so that the resolver marks those authentic servers as non-responsive. 

%The requirements for this attack are a combination of requirements for server poisoning (via NS or A RR), and then blocking the server, by destroying the authentic fragments.
Note that phase (2), i.e., server blocking, is not essential and the poisoning attack by itself implies NS hijacking. This is due to the fact that the TTL of the poisoned RR is higher than the TTL of the records cached from previous responses, therefore, once those authentic records expire from cache, the resolver will not request them and will use the poisoned cached NS RR.

As a result of this attack the resolver will only query the server of the attacker (as it is the only one that responds). However, the attacker cannot produce valid signatures for the records that it returns, and therefore it responds to resolver's queries with records that are not protected with DNSSEC. This attack has the `cache-or-crash' effect, i.e., the resolver will either cache those responses, or will timeout and not be able to provide responses (since this is the only name server that the resolver has for the victim domain). The response depends on the specific resolver in question, e.g., Unbound 1.4.1 in permissive mode caches such responses, while Bind9 times-out and does not.
%Therefore, resolvers that follow \cite{rfc4697,203}, are exposed to this attack.

%Note that the attack requires minimal efforts from the attacker - once it modified (just one!) IP address in the DNSSEC protected DNS response to its own address, and blocks the IPs of the other servers (effective for 15 minutes for Unbound) it has control over the victim domain from resolver's prespective, as the resolver will only query its server and will refrain from querying the real servers of the domain.



% a  server pinning, which does not rely on the behaviour recommended by \cite{rfc4697}, is to set long TTL (time to live) in the DNS records which the attacker adds to the DNS response. Note that this technique is limited only to responses where the attacker can replace all of the name server entries (in the {\tt authority} section), or all A RRs (in the {\tt additional} section), with his own. This is due to the fact that the resolver validates that all the NS records in the DNS response have the {\em same} TTL. Once the real name servers for the domain expire from cache, typically records for top level (and other popular) domains exist in the cache of the resolver, the resolver will be left with the attacker's servers which have significantly longer TTL. Since the resolver has servers for the target domain it will not request those records from the domain again, and will be rendered with attacker's servers.
\ignore{
\subsubsection{Cache-or-Crash Attacks} The resolver is rendered with only the IP of the server which the attacker selected. If the server entry is poisoned, i.e., the resolver cached a malicious IP address of the attacker,  then the responses from the server are not signed. The resolver can either fall back to a non-validating mode and accept the malicious responses (`cache'), or not provide DNS functionality for that domain, resulting in denial of service (`crash').

\subsection{Applications}\label{sc:app:pin}
Name server pinning and poisoned name server pinning can be exploited in several ways, creating significant new threats. We now briefly suggest some of these exploits and threats: 
\begin{description}
	\item [Covert Channel Attacks:] Botnets, i.e., networks of `bots' (adversary-controlled hosts), are one of the most critical security threat. One of the important mechanisms to detect bots, is via their communication (with other bots, command and control center, etc.). To evade detection, the bot can issue DNS requests to a seemingly legitimate domain, e.g., {\sf mil}. By using poisoned server pinning, the attacker can make a machine controlled by him the main name server for some victim domain, and then communicate by specially crafted DNS queries. The command and control center is the destination of that communication. However, even a regular server pinning (without poisoning) can suffice, in cases where attacker is a MitM on the route to the pinned name server, or can use side-channel such as IP-ID to communicate via the server. 
	
	\item [Traffic Analysis] Server pinning allows to redirect the traffic to the server of attacker's choice. If the attacker poisoned the entry for that server mapping it to its own IP address, than the attacker can also inspect all the DNS requests to the target domain (and as a result, also learn, e.g., the web sites that clients visit). In other cases, attacker may be able to utilize a side channel of the name server, such as IP-ID, to estimate the trafic from the resolver to the victim zone. 
	
	\item [Cache-or-Crash Attacks] The resolver is rendered with only the IP of the server which the attacker selected. If the server entry is poisoned, i.e., the resolver cached a malicious IP address of the attacker,  then the responses from the server are not signed. The resolver can either fall back to a non-validating mode and accept the malicious responses (`cache'), or not provide DNS functionality for that domain, resulting in denial of service (`crash').
\end{description}
}

\ignore{
%\subsection{DNS Poisoning Variants}
Exploiting Second-Fragment Overwriting for cache poisoning is non trivial. One challenge is that the response packet must be long enough to be fragmented, furthermore, the second fragment should contain sufficient part of the response, to allow attacker to inject a useful false (`poisonous') packet into the cache. 

Another challenge is to cause a meaningful poisoning. Recall that fragmentation happens (almost always) for responses to queries for resources within DNSSEC protected domains, e.g., {\sf gov}. Therefore, the impact of our second-fragment overwriting attack depends on the deployment of DNSSEC by zones and validation of DNSSEC by resolvers. We now describe the optimal attack strategies, i.e., which records to spoof in the second fragment, and the potential applications of poisoning such DNSSEC-enabled DNS responses, and map them to the requirements and attacks in Table~\ref{attacks:table}. Then, in Section~\ref{sc:dnskey}, we show an experimental evaluation of an attack poisoning a name server for {\sf org} domain; this attack is effective when the resolver is supporting a permissive operation mode, and allows to hijack the victim domain. The attack also works if the DNSSEC is correctly deployed, and can be used in tandem with name server pinning (Section~\ref{sc:ip}).
}
%that the attacker should follow based on the how variations of DNSSEC deployment can be exploited by attacker possible impact of our DNS cache poisoning attack 
%We also define each type of deployment status in corresponding sections below.
\ignore{
\subsubsection*{Permissive resolver.} A permissive resolver is one that supports DNSSEC, however, ignores DNSSEC validation failures. Obviously, for such resolvers, DNSSEC does not provide added security; yet, there appears to be a significant number of such resolvers~\cite{olafur:nat:res,castro2010understanding}, apparently due to concerns about loss of connectivity due to interoperability and other problems upon enforcing DNSSEC; see discussion in Appendix~\ref{sc:reqs}. Such implementors deploy DNSSEC incorrectly or possibly via an `incremental deployment', aiming to preserve DNS functionality with intermediate Internet devices, e.g., firewalls, and legacy resolvers which may discard DNSSEC enabled DNS responses or strip DNSSEC signatures. This approach apparently assumes that permissive use of DNSSEC can provide evidence on whether the network can deploy DNSSEC fully without problems or not, while not {\em harming} their security; unfortunately, this is not the case and such resolvers are open to poisoning. 

This allows the attacker to add a new name server for existing domain or to change an IP of existing name server; changing the IP (A RR) or the name server (NS RR) depends on the fragmentation, i.e., whether the {\tt authority} or {\tt additional} sections appear in the second fragment. This attack the same effect as the original Kaminsky cache poisoning attack \cite{kaminsky:dns}, and allows an attacker to hijack the victim domain.

\subsubsection*{Island of Security.} When the parent zone returns an NSEC or NSEC3 (indicating that the child does not support DNSSEC), while the child does (requirement 1. in Table~\ref{attacks:table}), the resolver cannot establish a `chain-of-trust' to the target zone and thus cannot validate the DNSKEY of the zone. This holds for many second level domains, e.g., children of {\sf gov} TLD (Figure~\ref{fig:subs-of-gov}), and even for some TLDs, e.g., {\sf mil}. As a result, the resolver falls back to non-validating mode, and ignores the signatures in a DNS response. an `island of security' (i.e., whose public key the resolver cannot validate).
The non-validating mode is identical to the `permissive resolver', and allows the attacker to add a new name server for existing domain (or change IP address of existing server).
}

% Both of these cases are not `proper' use of DNSSEC, yet they are highly frequent; we discuss this in more detail in Appendix~\ref{sc:reqs}. In this case, we can poison DNS responses by creating new name servers for {\em existing} domains; this attack has the same effect as the original Kaminsky cache poisoning attack \cite{kaminsky:dns} which poisoned resolver's cache with malicious records for real domains.

%\begin{definition}[Permissive Resolver (PR) or no DS]\label{def:permissive} A resolver accepts and caches a DNS response, even if the DNS records cannot be validated, e.g., due to missing signatures or keys or incomplete chain of trust (due to missing DS).
%\end{definition}

\ignore{
\subsubsection*{No Deployment of DNSSEC in Zone or Resolver.} 
This type of attacks is less challenging, albeit extremely dangerous when applicable; the attacks require that DNS responses get fragmented. The technique is rather straight forward, and the outcome is essentially equivalent to Kaminsky attack~\cite{kaminsky:dns}, i.e., the attacker adds a new name server (or maps an existing name server to the malicious IP) and therefore hijacks the whole victim domain; we model the requirements for these attacks in Table~\ref{attacks:table}, `Domain Hijacking' column.

If the target domain does not deploy DNSSEC and does not have long DNS records, e.g., {\tt TXT}, then our poisoning attacks are not applicable, since the DNS response will not result in fragmentation. Some name servers are susceptible to path MTU reduction, by spoofed ICMP packets\footnote{Not all operating systems reduce MTU upon receipt of such ICMP fragmentation needed packets. We validated and confirmed path MTU reduction technique against Linux Kernel 2.6 OS.}, which we suggest to use to cause fragmentation of DNS responses. Note that this technique is not always applicable, since many firewalls may be filtering such ICMP packets (with type:3, code:4), contrary to the recommendations of \cite{rfc1191}. Thus to be able to use path MTU reduction the attacker must ensure that no filtering is applied to its outbound packets, e.g., by its ISP, and the attack will fail if incoming traffic to the name server is subject to such filtering. The idea of spoofing ICMP fragmentation needed packets is not new and was suggested as an attack vector for denial of service attacks, \cite{icmp:dos,icmp:tcp:dos}, however it was not applied to cause fragmentation to DNS responses. 
%; we describe those techniques in Appendix~\ref{sc:icmp}. % If DNS responses get fragmented, then the attacker can retreat to creating arbitrary, poisonous responses, which adhere to the caching rules of the resolvers~\cite{son2010hitchhiker}; the result of the attack is essentially equivalent to adding a new name server (Kaminsky~\cite{kaminsky:dns}) and thus hijacking the domain.

Our second-fragment overwriting attacks are applicable even if the resolver does not support DNSSEC, but the victim domain does. This is due to the fact that if the attacker can trigger an arbitrary DNS query at the resolver, e.g., DNSKEY, then the resolver will query the appropriate name server, asking for those records. The responses from the server for those specific queries can often get fragmented, which allows our second-fragment overwriting attacks.
}
%
%  then the attacker can retreat to creating arbitrary, poisonous responses, which adhere to the caching rules of the resolvers~\cite{son2010hitchhiker}. Note this may be that even if the resolver does not support DNSSEC, the 
\ignore{
\subsubsection*{Correct DNSSEC Deployment.} We show vulnerabilities assuming that the zone correctly deploys DNSSEC and the resolver performs strict validation of DNSSEC enabled records. Resource records in the answer section of such domains are signed, hence, if the resolver performs strict validation of DNSSEC, it should not accept unsigned records in the answer section.
%\begin{definition}[Correct DNSSEC Deployment]\label{def:correct} The resolver is able to etablish a chain of trust from the root to the parent domain, and to validate the DNSKEY record of the target domain.
%\end{definition}

In contrast, the delegation records, NS (name server) and A (IP address), located in {\tt authority} and {\tt additional} sections, are not signed, see \cite{rfc4035}. This allows the attacker to change the IP address (in the {\tt additional section}) of the name server of some victim domain, to its own address, or to add a new name server for the victim domain. Such NS and A records are usually cached and used, for queries to the specified domain; see \cite{son2010hitchhiker}. At this point, the attacker managed to cause queries for the victim subdomain to be sent to a machine controlled by the attacker. %;  

This vulnerability, of redirecting DNSSEC enabled DNS requests to malicious server by a man-in-the-middle, was pointed out by Bernstein~\cite{Bernstein:woot}, yet without a specific application for such an exploit. Indeed, \cite{bau2010security} refute Bernstein's claim of this being a vulnerability, by proving that it does not enable the man-in-the-middle attacker any additional capabilities, and conclude that it does not pose a significant threat. Indeed, not signing the delegation records does not break the design requirements defined for DNSSEC, \cite{rfc4035}. Yet, we show that by applying our technique an off-path attacker can pin the name server (Section~\ref{sc:fix}) for a victim domain, can then perform a range of attacks including: traffic analysis, covert channel attacks, denial of service attacks.

The attacker can also create a new subdomain, e.g., {\sf secure.bank.com} under {\sf bank.com}, by creating an NS record (in the authority section) for the new subdomain {\sf secure.bank.com} mapping it to the name server which the attacker controls; this is modelled in column `New Subbdomain' in Table~\ref{attacks:table}.
This attack is only applicable to protected domains that use NSEC3 opt-out: the attacker may be able to use legitimate NSEC3 responses (for non-existing sub-domain), and turn them into what appears to be a legitimate referral to an unprotected sub-domain; this can be used for phishing attacks. Furthermore, as \cite{bau2010security} show, domains which deploy NSEC3 opt-out records are vulnerable to browser cookie theft by a man-in-the-middle attacker, as they allow the attacker to insert insecure delegations into DNS responses. This is in contrast to the recommendations in \cite{rfc5155} which suggest that NSEC3 opt-out does not pose a significant threat. Using our techniques an {\em off-path} spoofing attacker can perpetrate such attacks.
% . using our techniques allows an off-path attacker to steal browser cookie; this attack was outlined in \cite{bau2010security}, on domains which deploy NSEC3 opt-out records, but we use a weaker off-path attacker (and not a man-in-the-middle). As \cite{bau2010security} showed, NSEC3 opt-out enables the attacker to convert an insecure delegation to an unauthenticated denial-of-existence (and vice-versa), simply by changing the records in a DNS response. They show that converting the DNS response: (1) from insecure delegation to denial-of-existence can be used for denial-of-service attacks on resolvers (which cache these records), and (2) coverting a denial-of-existence to insecure delegation enables the attacker to insert an insecure delegation, and show that this can be used for browser cookie stealing.
%It is, however, possible to create fake {\tt authority} NS (or fake {\tt additional} `glue') records in a response. Such NS records are usually cached and used, for queries to the specified domain; see \cite{son2010hitchhiker}. At this point, the attacker managed to cause queries for the victim subdomain to be sent to a machine controlled by the attacker. Intuitively, it may seem that this does not `buy' the attacker anything, as it cannot forge subsequent responses from that new name server (or IP); indeed this was also the justification of \cite{rfc4033,4034,4035} for not signing these records, furthermore \cite{bau2010security} also assume that this forgery does not add any capabilities for the attacker and concluded that it does not create additional exploitable attacks. 
%Yet, we show that this can be used as a building block for a range of attacks, in particular, for name server hijacking. This attack validates the concern that was raised by Bernstein~\cite{Bernstein:woot} regarding a vulnerability of DNSSEC, which allows man-in-the-middle attackers to forge glue NS and A records within DNSSEC enabled-packets.
%, we can only change NS or A records (which are not signed by the DNSSEC).
%  (e.g., to add a new server for the domain name)   (to change the IP address of the existing server)

}

\ignore{
\subsection{Spoofing Name Server IP\\For Domain Hijacking}\label{sc:dnskey}
We present the attack flow in message exchange diagram, Figure~\ref{fig:org:attack}, for the case where the attacker applies fragment reassembly modification to spoof the IP for the name server of {\sf org} domain; Table~\ref{attacks:table}, `Domain Hijacking' (New IP).
This attack can have two impacts: (1) If the resolver does not perform strict DNSSEC validation (or if the domain were an island of security), then the attacker can hijack the the name servers for {\sf org} domain hijaking all of {\sf org's} subdomains. The impact of this attack is effectively equivalent to the Kaminsky poisoning attack. Yet it is practical as it circumvents all the defenses against Kaminsky attack, e.g., source port randomisation. (2) In contrast, if the resolver performs strict validation of the DNSSEC responses, then the attacker can perform `server-pinning' by applying the technique in Section~\ref{sc:ip} and blocking the rest of the name servers of {\sf org}.%; this can be useful, e.g., for traffic analysis or covert communication, when DNSSEC is correctly deployed.

The attacker triggers a DNS request via the usual techniques, e.g., via a malicious script~\cite{kaminsky:dns}, and then sends a spoofed second fragment to the resolver. In Figure~\ref{fig:org:attack} the resolver issues a DNS request for the DNSKEY of {\sf org}; this is an indirect way to trigger a query, i.e., the resolver asks for the DNSKEY of some domain automatically, when the DNSKEY expires from cache, or when it needs to validate records for that domain, e.g., to be able to validate an A record or a non-existing domain (NSEC3) record.
\begin{figure}[!ht]
\begin{center}
\fbox{
    \epsfig{scale=0.33,file=org-ns}
     }
\end{center}
\caption{\footnotesize{DNS poisoning attack of name server IP of {\sf org} domain. The resolver issues a query for a DNSKEY (e.g., when it expires from cache, 15 minutes for {\sf org}), and the spoofer sends a poisoned second fragment containing the forged entries of ORG. The query for DNSKEY of {\sf org} can also be triggered indirectly by issuing a query for non-existing (or for some other) domain within {\sf org}.}}
 \label{fig:org:attack}
\end{figure}

The annotated screen caption, Fig. \ref{fig:forged:resp:info}, presents the outcome of the attack. The first line (122) contains the `forged second fragment'; this fragment is kept in the defragmentation cache of the resolver, waiting for a matching first fragment (i.e., with the same set of {\tt (source IP=199.249.112.1, dest IP=132.70.6.202, fragment ID=7c6e, protocol=UDP)}). 

In the next line (133), we find the DNS query sent to the name server. This is a DNSKEY query sent to the (name server of the) {\sf org} top-level domain. Note that the DNSKEY query is issued automatically by DNSSEC-complying resolvers, e.g., as part of handling other queries; an attacker may also be able to cause a resolver, which does not support DNSSEC, to issue such a query, by sending an appropriate request to the resolver. 

Next line (134) is the first fragment of authentic response to the query, sent by the name server of {\sf org} (at IP 199.249.112.1). This response matches the fake second fragment already in the defragmentation cache, hence it appears as a complete DNS response packet. The contents of this packet are described in the lower panes; in particular, see the two forged resource records in the additional section, which contain incorrect (adversarial) IP addresses for two of the name servers  of the {\sf org} domain. In many cases, these records would be entered into the cache of the resolver (we discuss the conditions for this later on). 

Finally, notice that the authentic second fragment, received in line 135, has no matching first fragment (since the one received was already reassembled with the spoofed second fragment). Hence, it is entered into the defragmentation cache, where it is likely to remain until discarded (typically, after maximal lifetime of about 30 seconds). 
\begin{figure*}[!ht]
\begin{center}
\fbox{
    \epsfig{scale=0.45,file=fake-org-ns}
     }
\end{center}
\caption{\footnotesize{A Wireshark capture presenting the DNS packets in a DNS cache poisoning attack exploiting fragmented DNS responses by spoofing the second fragment of the response to the DNSKEY query; messages exhange diagram corresponding to this caption is in Figure~\ref{fig:org:attack}. %This attack works against DNS resolvers that do not perform strict validation of DNSSEC.
%Forged DNS response containing two A RR inserted by the attacker.
}}
\label{fig:forged:resp:info}
\end{figure*}
}

%\subsection{Experimental Evaluation}

 
%We tested this attack against a standard Unbound 1.4.1 resolver which supports two modes: (1) strict DNSSEC validation, and (2) permissive DNSSEC validation, whereby it accepts the responses even if some signatures are missing. The second (permissive) mode, allows to hijack the {\tt org} domain (once the attacker spoofs the IP addresses of the DNS servers authoritative for {\tt org}) and as a result to also hijack all of {\tt org} subdomains, e.g., {\tt iana.org}.%, that are also protected with DNSSEC.


==> randomip.tex <==
\subsection{Name-Server Blocking}\label{sc:ns:selection} \label{sc:ns:coercion} \label{sc:ip}\label{sc:block}\label{sc:fix} \label{ss:ns:blocking}\label{ss:removal}
In this subsection, we present the NS-blocking attack, allowing an off-path attacker to dissuade resolvers from querying particular name server(s); this can have multiple goals, including denial/degradation of service, traffic analysis and more (see next subsection). 

As indicated in Table \ref{attacks:table}, the NS-blocking attack has two main requirements: the ability of the attacker to generate a DNS query from the resolver, that will result in fragmented response from the `victim' name server; and that the resolver follows a behaviour recommended in RFC 4697 \cite{rfc4697,203}, namely, of avoiding a name server if there are two or more failures within some time interval (the time interval depends on the resolver implementation). We first describe how the attacker is able to block responses to a particular query, which does not rely on the behaviour recommended in \cite{rfc4697}.

%We present a techniques which enables the attacker to force a resolver to query the name server of attacker's choice. %, thus essentially `hijacking' the name server for the victim domain, from resolver's perspective. 
%\subsection{Exploiting Resolver Specific Behaviour}
%When zone operators employ multiple authority servers, the resolver should send the query to the one with the shortest response time, and avoid querying non-responsive name servers, see \cite{rfc1034,rfc4697}. However, there are no instructions on how to implement the server selection algorithm; as a result different resolvers, and even different versions thereof, implement different server selection algorithms, often resulting in inefficient implementations, \cite{203}.\\
%\subsection{NS Pinning by Blocking DNS Responses} 

%The fragment reassembly modification technique can be applied to perform the {\em Response-Blocking Attack}. 
To block responses to a query from a particular name server to the resolver, the attacker needs to send an arbitrary fake second fragment $y'_2$ with the anticipated IP-ID and other parameters, to match a legitimate response, as described above. The reassembly process using the legitimate first packet and the fake second fragment usually fails, and both fragments are silently dropped, by the UDP layer or by the DNS resolver itself, due to incorrect checksum. The resolver will resend the query after a timeout, but the timeout periods are known to the attacker, who can easily send appropriate fake fragments to cause loss of each of the responses, until the resolver gives up. The number of attempted retransmissions depends on the number of name servers that the zone uses; if the zone uses one name server, the resolver gives up in about 5 to 7 retransmissions, e.g., Bind9 after 7 timeouts, and Unbound 1.4.10 after 5 timeouts, if the zone uses more name servers then after one to two timeouts the resolver queries the next name server.

We show how to apply this technique, in order to perform NS-blocking, i.e., block a specific name server, instead of blocking just one particular packet. For this, we need the assumption that the resolver avoids querying unresponsive name servers, as per the recommendations in \cite{rfc4697,203}. We exploit the fact that when the target name server is not responsive, i.e., two or few queries times-out, the resolver does not send\footnote{Resolvers may send periodical probes, to detect when the target server becomes responsive, however, the period is so long that we can ignore it, e.g., for the Unbound name server, the period is 15 minutes. A similar behaviour of avoiding non-responsive name servers was observed by \cite{203} in PowerDNS and WindowsDNS.} any more queries to it. 
  %; this provides a sufficient `window' to launch the cache poisoning attack combined with the port derandomisation techniques (described in Section~\ref{sc:ttp}) for scenarios where the resolver located behind one of the NAT devices that we tested in this work.
 
\begin{figure*}[!ht]
\vspace{-15pt}
	\begin{center}
%	\fbox{
			    \epsfig{scale=0.35,file=ipderand-404gov}
%	     }
	\end{center}
\caption{\scriptsize{The Name-Server blocking attacks.}}
\label{fig:derand:ips} 
\vspace{-10pt}
\end{figure*} 
 
The attack is illustrated in Figure \ref{fig:derand:ips}. 
The idea is for the attacker to send a spoofed fragment, e.g., one byte long, which ruins the DNS response from the specific IP address. After repeating the attack few times (depending on the resolver software), e.g., twice in every 15 minute interval for Unbound, the resolver marks the name server (or rather the IP of the name server) as non-responsive and does not send queries to it for the specified interval of time which depends on the resolver implementation. %Note that this attack does not require any records in second fragment, and any size fragments, e.g., one byte long, suffice for attack to be effective.

It is important to notice, that with most resolvers, NS-blocking is effective against a specific {\em name server IP}, and not limited to a specific domain. Namely, we can use  NS-blocking to dissuade a resolver from using a specific name server, e.g., at IP address $38.103.2.1$, using queries (with fragmented responses) to one domain {\sf isi-sns.info}, and as a result the resolver will also avoid this name server for all the other domains which that server serves, e.g., {\sf paypal.com}. This can be very useful, as name servers often host multiple domains, and some of these may use DNSSEC (and have fragmented responses), or be owned (or corrupted) by the attacker (who can put some other record with fragmented response), while others may only have short (unfragmented) responses, in addition, some domains are much less frequently queried, e.g., {\sf info}, than popular domains, e.g., {\sf paypal.com}, that use the same name server, allowing to match the IP-ID with little effort; e.g., \cite{ramasubramanian2005perils} show that a typical domain name depends on 46 name servers on average which also serve other domains. 
 
%This technique is rather devastating, while requiring the attacker to expend minimal efforts for it to work. In particular, the increased use of load balancing, anycast~\cite{rfc3258}, and other mechanisms, allow more than one DNS server to share a single IP address. Therefore, by blocking one IP address the attacker effectively blocks a set of name servers. 

%The idea of destination IP prediction phase, in Figure~\ref{fig:derand:ips}, is to exploit large DNS responses which result in fragmentation; name servers that use TCP when responses exceed some predefined size, e.g., {\tt com}, are not susceptible to this attack. 

As illustrated in Figure \ref{fig:derand:ips}, we performed the attack against a {\sf 404.gov} domain, whose {\em non-existing domain} responses exceed 1500 bytes and thus get fragmented en-route. %; for simplicity in Figure~\ref{fig:derand:ips} we illustrate two servers instead of six.
This phase, of forcing the resolver to use a specific IP, requires a puppet, i.e., a script confined in a browser, which issues DNS requests via the local caching DNS resolver, at IP 1.2.3.4 in Figure~\ref{fig:derand:ips}.

In steps 1 and 2 the puppet coordinates with the attacker and issues a DNS request for {\sf \$123.404.gov} (where \$123 is a random prefix). In steps 3 and 4, the spoofer sends a forged second fragment, for all the possible name servers (i.e., a total of 2 spoofed fragments) except one which the attacker wants the resolver to use for its queries during the poisoning phase; the {\sf 404.gov} domain has three name servers. This ensures that only one IP address will result in a valid response, and the other two result in a malformed DNS packets. The spoofed second fragment is incorrect, and contains a single arbitrary byte (in addition to headers). In step 5, the spoofed second fragment is reconstructed with the authentic first fragment resulting in a malformed DNS packet which leaves the fragments reassembly buffer. This malformed DNS response is then discarded by the resolver, and the IP of the name server is marked\footnote{In reality the resolver marks the server as `non-responsive' after two unsuccessful responses; this is handled by sending two spoofed fragments with consecutive IP-ID in IP headers.} as `non-responsive'. When the authentic second fragment arrives, it does not have a match and is discarded after a timeout. As a result the resolver does not receive the response, and after a timeout it resends the DNS request to the next DNS server, step 6. The same procedure applies here, and the response is discarded. In step 9 a valid response arrives from IP 162.138.183.11. 
%In a real attack the resolver sends two queries to each server and marks the name server as non-responsive when {\em two} queries to that server result in a timeout; for simplicity in Figure~\ref{fig:derand:ips} we present the process for one query to each server. 
This way, by wrecking the responses from all name servers except one, we forced the resolver to direct all its queries for {\sf 404.gov} domain to 162.138.183.11.

The IP-ID allocation algorithm does not have a significant impact on our attacks against such resolvers (e.g., Unbound), since `misses', i.e., valid responses arriving to the resolver from some IP, do not prevent the attack; e.g., two failed (timed-out) queries suffice for Unbound to mark the server as non-responsive for 15 minute interval.

\indent The Wireshark capture, in Figure~\ref{fig:derand:wire}, that was run on the resolver, demonstrates the experimental evalutation, i.e., the DNS packets entering/leaving the network card of the resolver. During the course of the experiment the puppet issued 6000 queries\footnote{Note that our goal was to test the behaviour of the resolver, and to check the frequency of the queries to non-responsive servers; in real attack, once the IP-ID is known it is sufficient to issue two queries to mark the server as non-responsive.} to the resolver. The spoofer initiates the attack by sending three spoofed fragments to each IP address except 162.138.183.11. For simplicity, the capture presents only the packets exchanged between the resolver and the name server of 404.gov at 162.138.191.23 (by adjusting a corresponding filter in wireshark); the complete capture contains queries/responses from other name servers too. Packets numbered 18-20 are the forged fragments sent by the spoofer, with sequentially incrementing IP-IDs. Then puppet triggers a DNS request, packet 29. The response from the name server contains two fragments, packets 33 and 34. The first fragment is reassembled with spoofed fragment 18, resulting in a malformed packet which is discarded by the resolver. 

The second fragment is discarded after a timeout. In packet 48 the resolver requests a public verification key of the 404.gov zone. The response contains three fragments 49-51; the first fragment is reconstructed with the spoofed fragment in packet 20, which also results in a malformed DNS response and is discarded. Note that this request, in packet 48, was sent at 19:28. Based on our tests it can be seen that when Unbound encounters a timeout twice for the same destination IP, it stops sending further packets to that destination for 15 minutes. Indeed, the next packet that is sent to that IP is packet number 6848, at time 19:43. The same scenario was observed with IP 162.138.191.11. The queries between 19:28 and 19:43 were sent only to 162.138.183.11, avoiding 162.138.191.11 and 162.183.191.23. Note that even if some of the responses (between packets 33 and 49) were valid and accepted by resolver, e.g., if they were not fragmented, it did not make a difference, and two timed-out responses in a 15 minute interval were sufficient for Unbound to stop querying those IP addresses; this fact shows that the success probability of the attack does not depend on the IP-ID selection mechanism.
% Here we did not address the IP-ID value, and we show it in full version (it is important for the attack) and due to lack of space, 
% to add details on experiment and the details are in full version.
% due to this variety we find it indicative to caution against relying on IP randomisation as a counter measure, as other attacks may be found.
%
%When a server is detected as unresponsive unbound sends a query to probe the server every 15 minutes. PowerDNS also sends very few queries to unresponsive servers; unresponsive server has to wait 3 minutes to be selected. Both unbound and PowerDNS take a long time to detect server recovery.
\begin{figure*}[!ht]
\vspace{-15pt}
	\begin{center}
	%\fbox{
			    \epsfig{scale=0.6,file=cap-19123}
	%     }
	\end{center}
\caption{\scriptsize{The wireshark capture of the attack, presenting only the packets exchanged between the name server 162.183.191.23 and the resolver. As can be observed, after two malformed responses the resolver refrains from sending further queries to that name server for 15 minutes. Fragmented packets are coloured in white, DNS requests in black, and reassembled DNS fragments in blue.}}
\label{fig:derand:wire} 
\vspace{-10pt}
\end{figure*} 

\subsection{NS-Blocking: Applications} \label{ss:removal:appl}
NS-blocking is rarely a goal by itself; more often, it can serve as a mechanism for other goals. We discuss three such goals: facilitation of DNS poisoning; degradation of service, and traffic analysis. 

%While NS-Blocking is a simple attack, it can has several important applications, which we next describe. 
%This is the first technique to allow `server pinning' and can be used to direct a resolver to query some vulnerable name server, e.g., to perpetrate cache poisoning attacks. 

%The first application of NS-blocking is to 
\paragraph{Facilitate DNS poisoning} In  \cite{ramasubramanian2005perils}, Ramasubramanian and Sirer conducted a survey showing that a typical domain name depends on 46 servers on average, and names belonging to countries depend on a few hundred servers. They note that compromising a server can lead to domain hijacks and postulate that it is possible to hijack $30\%$ of the domains in Yahoo and DMOZ.org directories; DNS servers are known to have vulnerabilities~\cite{khurshid2011improving,dns:vuln}. However, \cite{ramasubramanian2005perils} did not suggest a technique which can be used to force a resolver to query a specific name server. NS-blocking can provide exactly the necessary mechanism. 

Also note that NS-blocking can assist in other DNS cache poisoning attacks, including these in the next section of this paper, as it allows the attacker to reduce the number of servers that the resolver can query, possibly to only one. 

\paragraph{Off-path Degradation of Service} By blocking `good' name servers, an attacker can cause resolvers to send their traffic to specific, `bad' name servers. In particular, resolvers may resort to name servers with very high latency, causing unnecessary delays. Note that the zone administrators often deploy techniques to distribute the load between several physical servers sharing the same IP, e.g., using load balancing or Anycast~\cite{rfc3258}. Typically not all the name servers of a domain deploy such optimisations, e.g., 6 out of 13 root servers,~\cite{liu2007two}. Our technique allows the attacker to block those servers and to `force' the resolver to query a name server which does not support such load balancing.

\paragraph{Off-path Traffic Analysis and Covert Channel} Many names servers provide side-channels allowing an attacker to learn or estimate the rate of requests handled by the server. In particular, one simple and effective side-channel is the IP-ID used by the name server. 

We next show how an off-path attacker can use this side channel, in conjunction with NS-blocking, to estimate (analyse) the rate of requests from some resolver $r$, to a particular domain {\sf foo.bar}. NS-blocking can facilitate such off-path traffic analysis in several ways; as we later explain, this side-channel can even allow covert communication (between a bot using the resolver, and an attacker which is not controlling the name server). 

First consider the case that one (or more) of the name servers of {\sf foo.bar}, say {\sf ns.foo.bar}, is using {\em globally-incrementing IP-IDs} (this is common). By using NS-blocking, we can direct all or most of the DNS requests from $r$ to {\sf ns.foo.bar}; by periodically querying {\sf ns.foo.bar}, the attacker can measure the rate of progress of the IP-ID (and hence of responses sent by {\sf ns.foo.bar}). To further improve the measurement, the adversary may use NS-blocking to cause other major resolvers to avoid using {\sf ns.foo.bar}. 

This mechanism also allows {\em off-path covert channel}, between an agent, say a bot $b$, which can use the resolver $r$, and an off-path attacker $o$, which can make queries to the name server {\sf ns.foo.bar}. The bot can, e.g., encode information by signaling via the queries to {\sf ns.foo.bar} (or possibly, signaling using distinct queries to several domains, each mapped to a specific, distinct name server). The attacker can communicate to the bot by signaling via loss of DNS responses. 

The traffic analysis attack is applicable also if none of the name servers of {\sf foo.bar} use globally-incrementing IP-ID, provided at least one of them, say {\sf ns.foo.bar}, uses {\em per-destination incrementing IP-ID}. In this case, the attacker will also need the ability to use the resolver $r$, e.g., via a puppet (malware such as script, in a sandbox). Attacker will use the puppet to keep track of the IP-ID used by {\sf ns.foo.bar} to send packets to $r$. %; we use the method of \cite{GH:WOOT11}, adapted to detect IP-ID of fragments sent to a resolver.  



%\begin{wrapfigure}{r}{0.7\textwidth}
%\vspace{-25pt}
%\center
%\mbox{
%			    \epsfig{scale=0.45,file=cap-19123}
%}
%\caption{\scriptsize{The DNS server IP address prediction attacks: spoofing attacker crafts a forged second fragment that gets reassembled with the authentic first fragment and results in a malformed packet, which is discarded by the resolver.}}
%\label{fig:derand:wire} 
%\vspace{-15pt}
%\end{wrapfigure}
%\indent Note that crafting a forged second fragment that would get matched with the authentic first fragment requires a match with the identification field (IP-ID) in the IP header.
%According to \cite{rfc791,rfc4963} the fragments of a datagram are associated with each other by their protocol number, the value in their IP-ID field, and by the source/destination address pair. Therefore the attacker is required to hit the correct IP-ID value, which is used by the name server in its DNS response. Many domains, as well as 404.gov, use per-destination sequential incrementing IP-ID values (or even globally sequential incrementing IP-ID, e.g., Windows OS). Other domains (mainly top level domains and the root servers) increment the IP-ID value sequentially per-destination.\\
%; an interested reader is refered to \cite{GH:WOOT11} for efficient IP-ID exposure techniques.
%We identified three cases: (1) per-destination sequential IP-ID, (2) global sequential IP-ID, (3) other IP-ID selection\footnote{This }. Globally incrementing IP-ID is trivial to learn, and such systems are easiest to exploit, e.g., Windows operating systems. If the IP-ID is random the attacker can send a large number of spoofed fragments to increase the probability for a hit with the IP-ID in first authentic fragment. The limit on the number of spoofed fragments that the attacker can send is the IP-ID reassembly buffer\footnote{The receiver allocates a separate fragmentation reassembly buffer for each source IP address. Thus the attacker can spoof fragments with IPs from several name servers concurrently without reducing the probability for a hit with each authentic first fragment.}, e.g., in Linux systems the default value is 64 packets. However, this default value can be updated. In our attacks we set the reassembly buffer size to 1000 packets.
%
%Most domains use a per-destination incrementing IP-ID counter. This allows hitting the correct IP-ID more efficiently (details in full version), and does not require a large reassembly buffer.
%\subsection{Experimental Evaluation}

\ignore{
--------------------

This technique can be used by the attacker as a building block to launch more advanced and complex attacks, e.g., denial of service, traffic analysis whereby the attacker can learn destinations of the DNS requests, as covert channel attacks by bots that query victim name server and the attacker receives the queries instead. In Section~\ref{sc:fix} we show how to extend server-pinning, by using server blocking can be used in tandem with DNS response poisoning, to result in a `poisoned server pinning'. In a poisoned server pinning the attacker `forces' the resolver to use its own malicious servers, instead of the real name servers of the domain. We then present the applications for these new attacks, in Section~\ref{sc:app:pin}

Furthermore, our technique can be applied to direct the resolver to a compromised name server,~\cite{ramasubramanian2005perils}.

To ensure efficient and robust functionality of the DNS, it is recommended, \cite{rfc2182,rfc1034}, that each domain should deploy a number of name servers. We found that the majority of top level domains (TLDs) use 5 to 7 authority name servers, and important domains, e.g., {\sf com}, use 13 authority servers\footnote{The list of TLDs is taken from the list published by IANA~\cite{iana:ips}.}; see Figure~\ref{fig:num:ips}.
\begin{figure}[!ht]
	\begin{center}
	\fbox{
			    \epsfig{scale=0.450,file=TLDsList}
	     }
	\end{center}
\caption{\scriptsize{The number of IP addresses in use by Top Level Domains (TLDs).}}
\label{fig:num:ips} 
\end{figure}

} % end ignore

==> removal.tex <==
\section{Fragment Overwriting and NS-Blocking} \label{s:removal} %\label{sc:ns:selection}
In this section, we present the {\em Name Server blocking (NS-blocking) attack}, allowing attackers to cause resolvers to avoid querying a name server. This attack requires much weaker assumptions than the poisoning attacks, Section~\ref{sc:poisoning}, and only assumes that the responses get fragmented. Both NS-blocking and the poisoning attacks, rely on {\em Fragment Overwriting}. 

Fragment Overwriting, explained next, allows attackers to modify fragmented packets. In Section \ref{ss:removal} we explain how fragment overwriting allows an attacker to cause standard-conforming resolvers to avoid a particular name server, i.e., to perform NS-blocking. Then, in Section \ref{ss:removal:appl}, we discuss potential exploits of NS-blocking. 

\subsection{Fragment Overwriting}%:\\Second Fragment Poisoning Attacks}
\label{s:simple-attack}\label{s:open-resolver}
%\subsection{Fragment Reassembly Modification}
We now present a simple technique, allowing an attacker to replace (overwrite) second fragments of (fragmented) IP packets, in particular, of DNS responses sent to the resolver; this basic technique is applied in all of our attacks. 

%In this section we present the technique of {\em replacing second fragments} of DNS which we use as a building block for all the attacks that we present in this work. All our attacks require fragmented DNS responses, which happen when the DNS response is larger than the link's maximal transmission unit (MTU), e.g., 1500byte. The attacker performs {\em fragment reassembly modification}, %which allows the attacker to replace an authentic fragment of the DNS response with a spoofed fragment.
%\subsection{Fragment Reassembly Modification and Response-Blocking DoS attack} \label{DoS}
Suppose  the original packet has payload $x$, and, after fragmentation, it is sent as two IP packets $y_1, y_2$. Then, the defragmentation process, running at the resolver\footnote{Alternatively, defragmentation may happen and at intermediate device such as a firewall or NAT; there is no impact on the attack.} on inputs $<y_1,y_2>$ reproduces $x$. 

To overwrite the second fragment, the attacker sends a fake second fragment $y'_2$ so that it arrives at the defragmentation module {\em before} the authentic fragments $y_1, y_2$ of the DNS response. The defragmentation mechanism in the IP layer will cache $y'_2$, in anticipation of the rest of the packet. By default, an unmatched fragment is kept in the cache for 30 seconds or so, hence, `planting' such fake fragments is easy; we now explain how the attacker can  ensure a match with the original packet. Note that it is easy to adjust this technique for the (less common) case where fragments are sent in a reverse order: attacker removes the authentic second fragment $y_2$ from the reassembly buffer by sending an arbitrary $y'_1$ (whose validation fields match those of the $y_2$), and the rest is the same as above.

According to \cite{rfc791,rfc4963} the fragments of a datagram are associated with each other by their protocol number, the value in their IP-ID field, and by the source/destination IP address pair.
Thus both the first authentic fragment $y_1$ and the second spoofed fragment $y'_2$ must have the same destination IP address (of the resolver that sent the query), the same source IP address (of the responding DNS server), the same protocol field (UDP) and the same fragment identifier (IP-ID). In addition, the spoofed second fragment should have the correct offset (as in the authentic second fragment). The fragment reassembly process, applied to the pair $<y_1, y'_2>$, returns either a failure or a different packet $x'\neq x$.  

Matching most of these parameters is not difficult. In particular, path MTU changes infrequently, and can be found by attacker easily, e.g., by trace-route. In many scenarios, the resolver has a single, known IP address; zones typically have 6 IP addresses on average. The attacker may sometimes also have some knowledge on the likely name servers since the server selection algorithms of many resolvers can be predicted~\cite{203}, e.g., based on latency, and may even use our attacks to disable some name servers; in the worst case, the attacker can launch the attack for each name server in parallel. In this work we show techniques which often allow the attacker to simply block the name servers of its choice.

%For IP to reassemble the original first fragment $y_1$ with the fake second fragment $y'_2$, the two must match in the IP addresses, protocol (UDP) and IP-ID field; in addition, the offset of the second fragment must exactly match the end of the first fragment. 
%(assuming IP-ID is already known). Then, when $f_1$, the first authentic fragment of the DNS response packet, arrives at the defragmentation module, the IP layer will match it with $f'_2$ (the fake second fragment) and and deliver the combined {\em poisoning packet} $p'=f_1||f'_2$ to the UDP layer.
%\subsection{Fragment Reassembly Conditions}

%\subsection{Second-fragment Overwriting}
%We use the following technique in our attacks, to replace the second fragment of the response packet $p=f_1||f_2$ with a fake second fragment $f'_2\neq f_2$, resulting in delivery of an incorrect packet $p'=f_1||f'_2$.


 %Some very large resolvers, in particular, public, open resolvers (e.g., of Google), use multiple IP addresses; we are now conducting experiment to check how many addresses are likely to be used. 
%To improve defenses against DNS poisoning,~\cite{rfc5452} recommends that resolvers randomly select a DNS server from all known (e.g., returned by the parent domain) name servers of the target domain.
%The naive strategy is to send fake fragments for each of the possible DNS servers, or repeat the attack few times until the resolver selects a matching name server. In Section~\ref{sc:ip} we present a technique which allows to force the DNS resolver to query a name server of attacker's choice, thus allowing to `pin' the IP address of the target domain server.
% and rarely much higher; see results in \cite{paper by Dagon?}. 



It remains to ensure a match between the value of the fragment identifier (IP-ID) field in the fake fragment $y'_2$, and the IP-ID in the authentic fragment $y_1$ of the original response $x$. There are several possible options for IP-ID prediction, depending on the version of the IP protocol (IPv4 or IPv6), the method that the name server's OS uses to select IP-IDs, and on the receiver implementation. 

In the most common case the communication is over IPv4, where the IP-ID field is 16 bits; and the host performing the defragmentation process, i.e., the resolver or firewall, has cache of 64 (or more) fragments per particular <source IP, destination IP, protocol> combination; note that when more than 64 fragments (for the same tuple) arrive, the oldest fragment is evicted from cache and is replaced with the new one. Assuming that the attacker has no knowledge on the process according to which the IP-ID is incremented, and assuming the IP-ID in the packet and in the fake fragment are selected independently, it suffices for the attacker to send 64 spoofed second fragments, to ensure success probability of roughly $1/1000$ of replacing the second fragment of a packet in a {\em single} attempt. A much better probability of success (as we discuss next) can typically be achieved, however, even this attack can be sufficiently efficient for many scenarios. 

Most systems select the IP-ID sequentially. Of these, many use a single counter for all destinations (globally-sequential), as in Windows and by default in FreeBSD. Other systems, e.g., Linux, use {\em per-destination} IP-ID counters. In both of these cases, the attacker can efficiently predict the IP-ID, achieving high probability of success (certainly compared to $1/1000$). In particular, for globally-incrementing IP-ID, which appears to be more widely used, e.g., {\sf mil}, the attacker can simply learn the current value, and the rate of propagation, by querying the name server directly. The technique we use to achieve improved success probability in the case of per-destination IP-ID, is an improvement of the methods of \cite{GH:WOOT11}. These techniques ensure feasibility of the attack even for most implementations of IPv6, in spite of its use of 32-bits IP-ID field. 

%We identified two IP-ID allocation strategies which DNS servers use: (1) {\em globally sequential} assignment, e.g., {\tt int} top level domain (TLD) and (2) {\em per-destination sequential} assignment, e.g., {\tt mil} TLD. The attacker can find out the globally sequential incrementing IP-ID by simply querying the name server by himself, i.e., if the resolver queries the DNS server after that the DNS response to the resolver will have a subsequent (higher) IP-ID. To find the per-destination incrementing IP-ID the attacker can send packets containing different IP-IDs until it hits the IP-ID. %; we extend more on this in Section~\ref{cs:ipid}.





%Note that for the poisoning attacks, it may suffice to 
%The trivial, `brute-force' approach is to send many fragments with different IP-ID values, hoping one would match. This works, but at significant costs, since the IP-ID field is 16 bits long (32 bits in IPv6), hence, probability of guessing it by sending $n$ guesses is roughly $n\cdot 2^{-16}$. Furthermore, the number $n$ of concurrent guesses is bounded by the cap on number of cached fragments from same source and destination IP addresses, e.g., $64$ in current Linux release. Hence, in this common case, attacker has to send $64$ guesses and the probability of success is about $0.1\%$. This seems to rule out the effectiveness of this technique for DoS; the cost may still be reasonable for poisoning (see following subsections). 

%However, in many cases, a more efficient attack is possible, namely, attacker can predict the IP-ID. In fact, this is often easy, e.g., in some operating systems, e.g., Windows and some OpenBSD releases, where the IP-ID values are taken from a single, globally-incrementing counter. Furthermore, rather reliable prediction of the IP-ID values is also possible for Linux and other systems using per-destination IP-ID counters; see   \cite{GH:WOOT11} for solution requiring a requires a zombie who can use the resolver, or a DNS-specific variant we developed, which only requires a puppet (to be described in the full version). 

%The three attack variants address different scenarios and goals. 
\ignore{
\subsection{Applications}
In the next two sections, we descibe attacks using this technique:
%We next outline the attacks that we present in this work, which are based on {\em fragment reassembly modification} technique: 
\begin{description}
\item [DNS Response Poisoning] In Section~\ref{sc:poisoning} we apply Second-fragment Overwriting to poison DNS responses, by modifying records in DNS responses, and e.g., adding a new name server for existing domain, or creating a new subdomain.
	\item [Name Server (NS) Pinning] In Section~\ref{sc:ip} we show how attacker can block DNS responses from a name server. We then apply such blocking to `pin` the target name server, which the resolver will query, ruining IP address randomisation. Furthermore, our technique can be applied to direct the resolver to a compromised name server,~\cite{ramasubramanian2005perils}. We also suggest several other applications of such `server-pinning' attack, most notably, for poisoned name-server pinning, which forces the resolver to query only name servers which attacker controls.
\end{description}
The attacks and their requirements are also summarised in Table~\ref{attacks:table}.
 }
 %We conducted our attack against a standard conforming DNS resolver implementation: Unbound (1.4.1), which we show to be vulnerable to destination IP derandomisation. Note, that the derandomisation technique, which we present next, does not apply to some DNS implementations, e.g., DNSCache, which does not keep history of previous queries, and each time selects the target name server uniformly. Nonetheless, the conclusion is that standard resolvers are based on `vague' server selection algorithms, often without analysis or a proof of security, and thus may be exposed to this or other types of attacks. Therefore,
% It appears that relying on the DNS server IP address randomisation for additional entropy requires careful study of particular resolver in question.

% to emphasise that we introduce techniques and the poisoning is the same.
\ignore{
{\sc The forged packet $p'$ is a valid DNS response.} In order for the forged packet $p'$ to result in cache poisoning, it must constitute a valid DNS response. In particular, the {\em UDP checksum} of $p'$ must be correct, or it will be discarded by the UDP layer (or by the resolver itself). Attackers are often able to ensure high probability of a valid DNS response, e.g., by querying the name server in advance for the same resource record and learning the contents of the corresponding DNS response, including all contents in the second fragment. To match the UDP checksum the attacker has to ensure that the checksum of the forged fragment $f'_2$ is identical to the checksum of the authentic second fragment $f_2$; this is easy to do, e.g., by changing two resource records: one to create the forged record, and another to fix the checksum. Notice that attackers cannot add (or remove) resource records from any section of the response, since the DNS header contains the number of records in each section of the response.
%Forged packet should contain 

{\sc DNS-valid RR $r_f$ in response $p'$.}  The forged response packet $p'$ should contain (at least) one {\em fake} resource record $r_f$. Furthermore, $r_f$ must be {\em valid}, i.e., not rejected as non-conforming by the resolver. The set of valid records depends on the request, the section in which the record appears, the domain and the resolver. In particular, resolvers are likely to ignore records which are out-of-bailiwick, records in the `answer' section whose domain name and/or type differ from the query, records in the `authority' section which are not  referrals to a domain containing the query, and records in the `additional' section which are not providing address for valid records in the `authority' section. Finally, if the resolver enforces DNSSEC, then the forged record must pass DNSSEC validation too; in this case the attacker can only add delegation (NS or A) records for the child zone, which are not signed by the DNSSEC, \cite{rfc4035}.  However, most resolvers that support DNSSEC do not perform strict validation of DNSSEC, \cite{olafur:nat:res}.

{\sc Resolver must add $r_f$ to cache.} The response $r_f$ must satisfy the resolver-specific conditions for adding a resource record to the cache; these conditions also depend on existing (related) records in the cache. See \cite{son2010hitchhiker} for discussion and comparison of these conditions in several common resolver implementations. We tested the attacks against Bind9 and Unbound 1.4.10 resolvers, and slight variations of the attacks work against each of these resolvers.
}




==> requirements.tex <==
\section{Attacks Requirements}\label{sc:requirements}
In this section we describe the requirements of the different attacks that we introduce in this work. See Table \ref{attacks:table} for the requirements of each attack. Below, we dedicate one subsection to the \Rfz\ and \Rpz\ requirements, and another one to the  \Rdnssec\ requirement. We initiate with a brief description of three technical requirements: IP-ID, \Ropt\ and RFC 4697. 
\subsection{Technical Requirements}
The {\em IP-ID requirement} is that attackers have `reasonable' probability of success in guessing the IP-ID in the responses from the name servers. In IPv4, the IP-ID field consists of only 16 bits; considering that fragment reassembly can usually hold a significant number of fragments for specific senders, typically at least 64, this implies a good success probability even if attacker just guesses the IP-ID values. Furthermore, many systems, and in particular most name servers, authoritative for major TLD zones, e.g., {\sf mil}, use operating systems where IP-ID is generated sequentially, either globally (for all destinations) or with per-destination counters. In both cases, we can significantly improve the probability for a correct match. We optimised the IP-ID prediction, in the per-destination case, by adapting the technique of \cite{GH:WOOT11} to be used with resolver. Note that in IPv6, it is harder to predict the IP-ID, since it is 32 bits and is sent only in fragmented traffic; however, IPv6 specifically recommends the use of sequential IP-ID, and hence can be guessed with good chance of success. The bottom line is that the IP-ID requirement is almost always satisfied. 

The {\em \Ropt\ requirement} is that the zone uses NSEC3 DNSSEC record with opt-out option~\cite{rfc5155}. This 
%e \Ropt\ requirement is necessary only by our subdomain injection attack, described in Section \cite{sc:SubInj}, i.e., to 
allows attackers to create fake (non-existing) sub-domains, and thereby facilitate XSS, phishing and cookie stealing attacks. Sub-domain injection attack was proposed in \cite{bau2010security}, that carried it out by a MitM attacker. In fact, \cite{bau2010security}, also suggested that the attack could be carried out by an off-path attacker, assuming that {\em only} the transaction ID in DNS packets is randomised. However, this assumption does not hold for most DNS resolvers, as they (at the very least) support source port randomisation. %; furthermore, \cite{bau2010security} validated their attack using a MitM attacker only. 
In Section \ref{sc:SubInj} we show that such an attack can be effectively carried out by an off-path attacker, that does not intercept and inspect packets, and against patched DNS resolvers, i.e., supporting source port randomisation, IP randomisation and DNS query randomisation.

In spite of the publication of this potential abuse by MitM \cite{bau2010security}, NSEC3 opt-out is still widely used, and often even recommended, since it improves performance (esp. as long as DNSSEC is deployed only in small fraction of the domains). 

The {\em RFC 4697 requirement} is that resolvers adhere to (one of) the recommendations in RFC 4697 \cite{rfc4697,203}, specifically, that a resolver will refrain from sending queries to a name server after (few) failures, i.e., timeout queries, within a predefined time interval, and to {\em lame} name servers, i.e., those that provide DNS responses where (some of) the DNSSEC records, e.g., signatures, are missing or corrupted. 
We show in Section \ref{sc:ns:coercion} that this allows an attacker to cause resolvers to stop using specific name server(s), facilitating poisoning attacks, as well as other attacks, including off-path traffic analysis and covert channel attacks. We validated this behaviour in popular and standard DNS resolvers, see Section~\ref{sc:ns:selection}.

%All our attacks apply the second fragment overwriting technique to inject spoofed records into the DNS response, but differ in assumptions, which the attacks require. The difference is expressed in: (1) requirements on the {\em zone file} of the target (victim) domain and on the parent domain, (2) requirements on {\em resolvers}, and (3) requirements on {\em name servers}.

%The requirements on the zone file and name server are relevant to the feasibility of the attack. The requirements on the resolver allow optimisations to the attacks.

\subsection{Fragmentable Zone and Poisonable\\Zone Requirements} \label{sc:frag:req}
%\Rfz\ and \Rpz\ requirements} \label{sc:frag:req}
We now describe our two fragmentation requirements: \Rfz\ and \Rpz. 
The {\em\Rfz} requirement is necesssary to all of our attacks, and essentially amounts to the ability of the attacker to cause fragmentation of a response from a name server.
As can be seen in Figure \ref{fig:lengths-of-gov}, long second fragments are rather common, and responses are fragmented from most top level domains (which deploy DNSSEC), e.g., in the {\sf gov} top-level domain, which is the top-level domain with maximal adoption of DNSSEC so far. 

Note that fragmentation can also occur even if the resolver does not deploy DNSSEC, e.g., it relays a query for a DNSKEY from the client, or due to other types of records which can be long, e.g., different TXT records, and/or when fragmentation occurs at relatively low packet length $l$, due to success in sending fake ICMP fragmentation-required alerts (see Section \ref{sc:frag:req}).
\begin{figure}[!ht]
\begin{center}
%\fbox{
    \epsfig{scale=0.35,file=gov-all}
%     }
\end{center}
\caption{\footnotesize{Length of ANY and NXDOMAIN responses of {\sf gov} domains. Domains taken from \cite{gov:list}}}
 \label{fig:lengths-of-gov}
\end{figure}

 The {\em\Rpz} requirement is necessary for our poisoning attacks, and requires that at least one complete record is present in the second fragment so that the attacker can modify the second fragment and replace the authentic resource record with a spoofed one, which gets accepted and cached by the resolver. Details follow. 

The ability to cause the required fragmentation depends both on the records in the zone file, as well as on the properties of the name server (including the route from the name server to the resolver). In particular, fragmentation typically depends on the smallest MTU enroute on the path from the name server to the resolver; packets larger than 1500 bytes will normally be fragmented. The attacker may also sometimes be able to `trick' the name server into fragmenting (even) shorter packets before sending them. The attacker can inflict fragmentation by sending a spoofed ICMP `fragmentation needed' packet, similar to attacks in \cite{rfc5927}. Let $l$ denote the size of packets, above which attacker can cause fragmentation - the minimal MTU along the path, or the minimal length that the attacker can `force' the name server to use by issuing fake ICMP fragmentation-needed alerts. 

In principle, name servers could be configured to never allow fragmentation of responses, by sending response packets of length up to (some bound of) $l$ bytes with the DF (do not fragment) bit set, and send longer responses only via TCP, relying on TCP's path MTU discovery mechanism. However, the use of TCP for DNS requests and responses has significant performance penalty, in addition to the overhead and complexity of handling fragmentation-required ICMP alerts received due to sending packets with the DF set, which reach a network whose MTU is smaller than the packet size. Hence, we do not expect name servers to send packets with DF bit set (and indeed have not seen this behavior, e.g., {\sf com, edu}). 

Note that for the \Rfz\ requirement to hold, any fragmentation suffices, e.g., of 1 byte, and there is no requirement on the contents or length of the second fragments.  Hence, we only require existence of a response whose length is greater than $l$. 

%A complementing condition is that the attacker is able to generate appropriate responses, which can allow fragmentation.
A \Rpz\ requirement is a stronger assumption, since it also implies that the attacker is able to include a (fake) resource record in the response, such that the response - and in particular the fake record - would pass validation at the resolver and get cached. This requires that the second fragment is predictable\footnote{The (off-path) attacker can query the victim name server itself to select the query whose response it will poison.} (to allow attacker to avoid corrupting the checksum), and that it contains at least one modifiable record - typically, an NS record in the {\tt authority} section, or an A (`glue') record in the {\tt additional} section. The challenge here is mainly to find queries which will result in second fragments containing the necessary record(s) which the attacker will replace with its own. 

{\sc Caching and Time to Live (TTL).}
%Until this point,  we ignored the fact that 
The DNS resolvers will not issue queries at all, if there is a corresponding cached response. The TTL field of each DNS resource record indicates how long it may be cached by resolvers. 

The majority of TTLs of DNS records range between one hour to one day, \cite{jung2002dns}. However, many records have very low or even zero TTLs, e.g., records of content distribution networks (CDNs). Furthermore, some queries, most notably for non-existent domain, always or usually would not be in cache. In fact issuing queries for non-existent domain is similar to Kaminsky style attack, and allows to initiate the attack as frequently as required since the attacker simply prepends a new random string to the query. We demonstrated attacks exploiting fragmented {\em non-existent domain}\footnote{Non-existent domain DNS response contains an error bit in the DNS header, i.e., RCODE=`name error', and indicates that the requested name does not exists in the zone file.} or {\em no-data}\footnote{No data DNS response does not contain an error, i.e., RCODE=`no error', and it means that the requested name exists in the zone file but does not have the type requested in the DNS query.},~\cite{rfc2308}, DNSSEC-enabled responses.
We also found that often DNSSEC public verification key (DNSKEY) records, which typically exceed MTU and get fragmented, have relatively short TTL e.g., 15 minutes in {\sf org} domain; they also often indicate short expiration time in the signatures. 

Hence, caching would usually not prevent the attack, and the expiration time of some record from the cache can be anticipated by the attacker; there may be some impact on length of attack and possibly on its communication costs too, but this would not make the attack infeasible. Usually, successful poisoning happens within reasonable time. 

\subsection{\Rdnssec\  requirement}
The \Rdnssec\ requirement is that DNSSEC validation is either not used or is not {\em correctly} used, and thus ignored by the resolver; `Island' means that not {\em all} the zones from the root to the target zone deploy DNSSEC correctly, and `Permissive' means that resolver does not fail even DNSSEC-enabled responses do not validate. In either of this cases, DNSSEC does not offer protection, although deployed. %This holds for many second level domains, e.g., children of {\sf gov} TLD (Figure~\ref{fig:subs-of-gov}), and even for some TLDs, e.g., {\sf mil}. 

  %This holds in the common case, where DNSSED is not used by the resolver at all; however, in this case, it may be impossible or challenging to satisfy either of the fragmentation requirements (\Rpz\ and \Rfz), since fragmentation of DNS responses is usually due to DNSSEC resource records. Note that exceptions exist, with fragmentation of responses not containing DNSSEC resources; this may be due to other types of resources which can be long, e.g., different TXT records, and/or when fragmentation occurs at relatively low packet length $l$, due to success in sending fake ICMP fragmentation-required alerts (see Section \ref{sc:frag:req}).

\begin{figure}[!ht]
\begin{center}
%\fbox{
    \epsfig{scale=0.2,file=subdomains-gov}
 %    }
\end{center}
\caption{\footnotesize{The DNSSEC deployment, in the list from \cite{gov:list} of 1500  subdomains of {\sf gov}.}}
 \label{fig:subs-of-gov}
\end{figure}
%However, there are two common cases where \Rdnssec\ is satisfied, while the response are sufficiently long, and thus fragmented, due to the use of DNSSEC: (1) permissive resolvers and (2) island of security. However, in both cases, the protection of DNSSEC 
\paragraph{Permissive Resolvers.} A permissive resolver is one that supports DNSSEC, however, ignores DNSSEC validation failures, e.g., if the signatures are missing or invalid; Unbound DNS resolver has an explicit `permissive' mode to support such operation. Obviously, for such resolvers, DNSSEC does not provide added security; yet, there appears to be a significant number of such resolvers~\cite{olafur:nat:res,castro2010understanding}, apparently due to concerns about loss of connectivity due to interoperability and other problems upon enforcing DNSSEC. Such implementors deploy DNSSEC incorrectly or possibly via an `incremental deployment', aiming to preserve DNS functionality with intermediate Internet devices, e.g., firewalls, and legacy resolvers which may discard DNSSEC enabled DNS responses or strip DNSSEC signatures. This approach apparently assumes that permissive use of DNSSEC can provide evidence on whether the network can deploy DNSSEC fully without problems or not, while not {\em harming} their security; unfortunately, this is not the case and such resolvers are open to poisoning. 

\paragraph{Island of Security.} When the parent zone returns an NSEC or NSEC3 (indicating that the child does not support DNSSEC), while the child does, the resolver cannot establish a `chain-of-trust' to the target zone and thus cannot validate the DNSKEY of the zone. This holds for many second level domains, e.g., children of {\sf gov} TLD (Figure~\ref{fig:subs-of-gov}), and even for some TLDs, e.g., {\sf mil}. As a result, the resolver falls back to non-validating mode, and ignores the signatures in a DNS response. %an `island of security' (i.e., whose public key the resolver cannot validate).
%The non-validating mode is identical to the `permissive resolver', and allows the attacker to add a new name server for existing domain (or change IP address of existing server).

\ignore{
\begin{description}
	\item [Permissive resolvers] DNS resolver implementations that are willing to accept the DNS responses even when DNSSEC validation fails, e.g., if the signatures are missing or invalid; Unbound DNS resolver has an explicit `permissive' mode to support such operation. The support of `permissive' mode in resolvers is due to concerns about possible interoperability and hence availability problems if DNSSEC validation is enforced. Recent study \cite{olafur:nat:res} found that most resolvers that support DNSSEC, are permissive, i.e., do not perform strict validation of DNSSEC.
	\item [Islands of security] zones that deploy DNSSEC, but the resolver cannot establish a chain-of-trust to validate their DNSKEY records, since the parent zone does not provide a signed digest of the key of the child zone; note that `islands of security' is a frequent scenario, e.g., the root does not delegate the signed key of the TLD {\sf mil} domain, many of the children of {\sf org} TLD are also islands (although {\sf org} deploys DNSSEC). When the resolver cannot establish a chain of trust to the target zone and validate its DNSKEY, it falls back to the non-validating mode.
\end{description} 
}
%since the deployment of DNSSEC recently took off, the vast majority of zones are not yet signed. However, even zones that deploy DNSSEC, often do not do this correctly, and thus do not enable DNSSEC protection to clients. The reason is inherent in the complex structure and requirements of DNSSEC, e.g., the public verification keys of a zone need to be propagated to the parent zone (to enable the resolver to establish chain of trust), the keys need to be refreshed/revoked, the records need to be resigned when signatures expire. As a result of this complexity, implementation problems prone to occur. Indeed, many parent zones do not delegate the public verification keys for their DNSSEC enabled children, the child is an `island of security', i.e., rendered without DNSSEC protection.% These and other failures result in many `permissive resolvers' in order to prevent failures in DNS service, and to allow for an `incremental' deployment of DNSSEC.  Indeed, w


\ignore{

%%%%%%%%%%%% ZONE FILE %%%%%%%%%%%%

\subsection{Zone File Requirements}
The records that the zone file contains impact the control of the attacker: (1) over the queries which it triggers (response to which it wishes to poison), and (2) over the timing of the attack.

\subsubsection*{Time to Live (TTL)}
The TTL field of each DNS resource record indicates how long it may be cached. Some records have TTLs of zero, meaning do not cache, e.g., low TTL values are common in content distribution networks (CDNs)\footnote{CDNs use TTL-based DNS redirection service to balance the workload for Web sites.}. Majority of TTLs of DNS records range between one hour to to one day, \cite{jung2002dns}.

The TTL of a resource record imposes a ristriction on the frequency at which the attacker can trigger a DNS request for that record.

\subsubsection*{Resource Records (RRs)}
The mappings in DNS zone file are called resource records. The popular ones, and most relevant to our work, include: {\tt NS} (name server) records, {\tt A} (domain name to IP address mapping) records, {\tt MX} (mail exchangers) records. There are also DNSSEC specific records: {\tt nsec}, {\tt nsec3}, {\tt ds}, {\tt dnskey}.

%\subsubsection*{Number of Name Servers}


\subsubsection*{DNSSEC Deployment}
If the zone supports DNSSEC, and is not an island, i.e., the parent zone returns a DS record which can be used to validate the key of the child.

%%%%%%%%%%%% RESOLVER %%%%%%%%%%%%

\subsection{Resolvers}
\subsubsection*{DNSSEC Deployment}
Permissive or strict validator.
\subsubsection*{Server Selection Algorithm}
Queries non-responsive servers.

%%%%%%%%%%%% SERVER NS %%%%%%%%%%%%

\subsection{Name Server}
requirements on the network
\subsubsection*{Transmission Protocol}
Uses UDP or TCP for long responses.
\subsubsection*{IP-ID Assignment} 
Per-destination or global.
\subsubsection*{Response to ICMP Frag Needed}
\subsubsection*{MTU}
The minimal MTU on the path from the name server to the resolver.


\subsection{Poisoning Attacks}
\subsection{Attack 1}
frequency: the attacker can 
query

Attacker uses the same query 
Attacker can select any query and repeat the attack as frequently as it wishes. 
This requires NSEC3 responses 

\subsection{Attack 2}

\subsection{Attack 3}

%Bind 9.2.3
}



